Two- & Three-character solutions to MLDEs and Ramanujan-Eisenstein Identities for Fricke Groups

In this work we extend the study of arXiv:2210.07186 by investigating two- and three-character MLDEs for Fricke groups at prime levels. We have constructed these higher-character MLDEs by using a $\mathit{novel}$ Serre-Ramanujan type derivative operator which maps $k$-forms to $(k+2)$-forms in $\Gamma^{+}_0(p)$. We found that this $\mathit{novel}$ derivative construction enabled us to write down a general prescription for obtaining $\mathit{Ramanujan-Eisenstein}$ identities for these groups. We discovered several $\mathit{novel}$ single-, two-, and three-character admissible solutions for Fricke groups at levels $2$ and $3$ after solving the MLDEs among which we have realized some in terms of Mckay-Thompson series and others in terms of modular forms of the corresponding Hecke groups. Among these solutions, we have identified interesting non-trivial bilinear identities. Furthermore, we could construct $\mathit{putative}$ partition functions for these theories based on these bilinear pairings, which could have a range of lattice interpretations. We also present and discuss modular re-parameterization of MLDE and their solutions for Fricke groups of prime levels.

==> Fricke_2_MLDE.tex <==
\section{$\mathbf{\Gamma^{+}_0(2)}$}

\subsection{Riemann-Roch}
The valence formula for $\Gamma^{+}_0(2)$ reads \cite{2006math......7408M},
\begin{align}\label{valence_Fricke_2}
    \nu_{\infty}(f) + \frac{1}{2}\nu_{\tfrac{i}{\sqrt{2}}}(f) + \frac{1}{4}\nu_{\rho_{2}}(f) + \sum\limits_{\substack{p\in\Gamma_{0}^{+}(2)\backslash\mathbb{H}^{2}\\ p\neq \tfrac{i}{\sqrt{2}},\rho_{2}}}\nu_{p}(f) =   \frac{k}{8},
\end{align}
where $\rho_2 := \frac{-i+1}{2}$ and $\frac{i}{\sqrt{2}}$ is the Fricke involution point. From Proposition 3.1 of \cite{2006math......7408M}, we note that $E^{2+}_4$ has a zero at $\tau=\rho_2$ of order $2$ and $E^{2+}_6$ has a zero at $\tau=\rho_2$ of order $1$ and a zero at $\tau=\frac{i}{\sqrt{2}}$ of order 1.\\

The Riemann-Roch for $\Gamma^{+}_0(2)$ reads,
\begin{align}
    \sum_{i=0}^{n-1} \, \alpha_i = \frac{n(n-1)}{8} - \frac{\ell}{4}, \label{RR2}
\end{align}
where, $n$ is the number of linearly independent characters, $\alpha_i$s are exponents and $\ell$ is the wronskian index.

\subsection{The operator}
Consider the following transformations (where $\gamma\in\Gamma^{+}_0(2)$),
\begin{align}
    &2E_2(2\gamma\tau) = 2(c\tau+d)^2E_2(2\tau) + \frac{6c}{i\pi}(c\tau+d), \label{E22tau} \\
    &E_2(\gamma\tau) = (c\tau+d)^2E_2(\tau) + \frac{6c}{i\pi}(c\tau+d), \label{E2tau} \\
    \text{leading to,} \, \, &E_2^{2+}(\gamma\tau) = (c\tau+d)^2E_2^{2+}(\tau) + \frac{4c}{i\pi}(c\tau+d) \label{E22+tau}.
\end{align}
Eq.(\ref{E22+tau}) motivates us to define the following derivative operator in the space of $\Gamma^{+}_0(2)$, acting on weight $k$ forms,
\begin{align}
    \Tilde{D}_k := \Tilde{\partial}_\tau - \frac{k}{8}E_2^{2+}(\tau). \label{deriv_op}
\end{align}
where $\Tilde{\partial}_\tau := \frac{1}{2i\pi}\partial_\tau = q\partial_q$.
\\

One can check that for any modular form in $\Gamma^{+}_0(2)$, $\Tilde{D}_k$ maps $k$ forms to $k+2$ forms. Now if we construct the MLDE in the space of $\Gamma^{+}_0(2)$ withe the above derivative operator then the MLDE will be consistent with the Riemann-Roch formula for $\Gamma^{+}_0(2)$. However, if we use the usual \textit{Serre-Ramanujan} derivative to write down the MLDE in $\Gamma^{+}_0(2)$ then the resulting MLDE will not be consistent with the Riemann-Roch formula for $\Gamma^{+}_0(2)$.\\

Note that, if in a given space of modular forms there exists a weight $2$ form then the usual \textit{Serre-Ramanujan} derivative will work and the MLDE will remain consistent with the corresponding Riemann-Roch. This begs the question will we get two different MLDEs for spaces which have a weight 2 modular form? \\

We note below some interesting properties of the above derivative operator,
\begin{align}
    &\left(\Tilde{\partial}_{\tau} - \frac{1}{8}E_2^{2+}\right)E_2^{2+} = -\frac{1}{8}E_4^{2+}, \label{De2} \\
    &\Tilde{D}E_4^{2+} = -\frac{1}{2}E_6^{2+}, \label{De4} \\
    &\Tilde{D}E_6^{2+} = -\frac{3}{4}(E_4^{2+})^2 + 64\Delta_2, \label{De6},
\end{align}
where $\Delta_2(\tau)=(\eta(\tau)\eta(2\tau))^8=\frac{17}{1152}((E^{2+})^2-E_{8}^{2+})$ and $\eta(\tau)$ is the Dedekind-eta function.

\subsection{$j^{2+}$ plane}
Since, $q\partial_q\Delta_2 = E_2^{2+}\Delta_2$, we have the following relations,
\begin{align}
    &\Tilde{\partial}_\tau = -j^{2+}\frac{E_6^{2+}}{E_4^{2+}}\partial_{j^{2+}}, \label{j1_2} \\
    &\Tilde{D}^2_\tau = (j^{2+})^2\left(\frac{E_6^{2+}}{E_4^{2+}}\right)^2\partial^2_{j^{2+}} + \left(\frac{1}{2}j^{2+}\left(\frac{E_6^{2+}}{E_4^{2+}}\right)^2+\frac{3j^{2+}}{4}E_4^{2+}-64E_4^{2+}\right)\partial_{j^{2+}}. \label{j1_21}
\end{align}
We also have,
\begin{align}
    \frac{j^{2+}}{j^{2+}-256} = \frac{(E_4^{2+})^3}{(E_6^{2+})^2}. \label{re_F2}
\end{align} 
The above relation also shows,
\begin{align}
    &\lim\limits_{\tau\to\frac{i}{\sqrt{2}}} j^{2+}(\tau) = 256, \label{j2_1} \\
    &\lim\limits_{\tau\to\rho_2} j^{2+}(\tau) = 0, \label{j2_2} \\
    &\lim\limits_{\tau\to i\infty} j^{2+}(\tau) = \infty, \label{j2_3}
\end{align}
Using Eq.(\ref{j1_2}), (\ref{j1_21}) and (\ref{re_F2}) we can now recast $\tau$-plane MLDEs for $\Gamma^{+}_0(2)$ into $j^{2+}$-plane MLDEs. We shall derive Eq.(\ref{re_F2}) later in Sec. \ref{sec2}.

\subsection{$\mathbf{(1,\ell\neq 0)}$ MLDE}\label{sec1}
Let us do here some $1$-character computations. From Riemann-Roch we get that $c=6\ell$.
\\

$\ell=0$ is trivial so let us start with $\ell=1$. For $\ell=1$, the RHS of valence formula reads $\frac{1}{4}$ (since $k=2\ell$ always). The MLDE takes the following form,
\begin{align}
    \Tilde{D}\chi + \frac{1}{4}\left(\mu_1\frac{(E_4^{2+})^2}{E_6^{2+}}+\mu_2\frac{\Delta_2}{E_6^{2+}}\right)\chi = 0. \label{F2_l1_p1}
\end{align}
Now using the indicial equation we can set $\mu_1=1$. Now let us take a guess, $\chi=(j^{2+})^{\frac{1}{4}}$. One can readily check that this is a solution with $\mu_2=-256$. This solution will re-appear as a solution to a $(2,0)$ MLDE paired up with an unstable character.\\

Now let us analyse $\ell=2$. The MLDE takes the following form,
\begin{align}
    &\left(\Tilde{D}+\mu_1\frac{E_6^{2+}}{E_4^{2+}}\right)\chi = 0, \label{1char_F2_l2} \\
    &\left(E_4^{2+}\Tilde{D}+\mu_1E_6^{2+}\right)\chi = 0. \label{1char_F2_l2_aliter}
\end{align}
Note that in above $\Tilde{D}=q\partial_q$. Also, the indicial equation ($\alpha_0+\mu_1=0$) dictates $\mu_1=\frac{1}{2}$.
\\

Now let us take a guess, $\chi=(j^{2+})^{\frac{1}{2}}$. Then, $\Tilde{\partial}_\tau (j^{2+})^{\frac{1}{2}} = -\frac{1}{2}(j^{2+})^{\frac{1}{2}}\frac{E_6^{2+}}{E_4^{2+}}$. Note, that this $\chi$ indeed satisfies Eq.(\ref{1char_F2_l2}) with $\mu_1=\frac{1}{2}$.\\

Now let us do $\ell=3$. For $\ell=3$, the RHS of Valence Formula reads $\frac{3}{4}$ (since $k=2l$ always). The MLDE takes the following form,
\begin{align}
    \Tilde{D}\chi + \frac{1}{4}\left(\mu_1\frac{(E_4^{2+})^2}{E_6^{2+}}+\mu_2\frac{\Delta_2}{E_6^{2+}}\right)\chi = 0. \label{F2_l1_p1}
\end{align}
Now using the indicial equation we can set $\mu_1=3$. Now let us take a guess, $\chi=(j^{2+})^{\frac{3}{4}}$. One can readily check that this is a solution with $\mu_2=-768$.

Next let us consider the $\ell=4$ case. From the Riemann-Roch, we notice that this is the \textit{bulk-pole} MLDE. The MLDE takes the following form,
\begin{align}
    &\left(q\partial_q+\mu_1\frac{E_{10}^{2+}}{(E_4^{2+})^2+\mu_2\Delta_2}\right)\chi = 0, \label{1char_F2_l4} \\
    &\left(((E_4^{2+})^2+\mu_2\Delta_2)q\partial_q + \mu_1E_{10}^{2+}\right)\chi = 0. \label{1char_F2_l4_aliter}
\end{align}
The indicial equation dictates $\mu_1=1$. The recursion relation reads,
\begin{align}
    \sum\limits_{k=0}^i\left[(E_4^{2+})^2_{,k}m_{i-k}(i-k-1) + \mu_2\Delta_{2,k}m_{i-k}(i-k-1)+E_{10,k}m_{i-k}\right] = 0. \label{recurF2l42char}
\end{align}
Putting $i=1$ in Eq.(\ref{recurF2l42char}) gives,
\begin{align}
    m_1 = 104 + \mu_2, \label{m1eqn_F2_2char_l4}
\end{align}
which implies that $\mu_2\in\mathbb{Z}$. Now putting $i=2$ in Eq.(\ref{recurF2l42char}) yields,
\begin{align}
    m_2 = 4372. \label{m2eqn_F2_2char_l4}
\end{align}
One can check upto higher orders and check that,
\begin{align}
    \chi &= q^{-1}(1 + (104+\mathcal{N})q + 4372q^2 + 96256q^3 + 1240002q^4 + \mathcal{O}(q^5)) \nonumber\\
    &= j^{2+} + \mathcal{N} \, \, \, \, (\text{with} \, \mathcal{N}\geq -104)
\end{align}

\subsubsection{Tensor-Product formula}
Consider two different admissible $p$-character and $q$-character solutions. Let us say the Wronskian indices are $m$ and $n$ respectively. The tensor product solution will have $pq$ no. of characters and say its Wronskian index is $\Tilde{l}$, then,
\begin{align}
    \Tilde{l} = \frac{pq}{2}(p-1)(q-1) + pn + qm, \label{hampa_mukhi_tensor}
\end{align}
which is exactly similar to the \textit{Hampapura-Mukhi} formula for the $\text{SL}(2,\mathbb{Z})$ case (see \cite{Hampapura:2015cea}).\\

Using Eq.(\ref{hampa_mukhi_tensor}) we immediately note that, $((j^{2+})^{\frac{1}{4}})^{\otimes n}$ is a $(1,n)$ admissible solution.\\

Similarly, one can readily see that ${}^{(2)}\mathcal{W}\otimes((j^{2+})^{\frac{1}{4}})^{\otimes n}$ is a $(2,2n)$ admissible solution (where ${}^{(2)}\mathcal{W}$ is a $2$-character admissible solution). \\

Also, ${}^{(3)}\mathcal{W}\otimes((j^{2+})^{\frac{1}{4}})^{\otimes n}$ is a $(3,3n)$ admissible solution (where ${}^{(3)}\mathcal{W}$ is a $3$-character admissible solution). \\

Note that, the most general single-character solution can be written as, (with $c=6N$ and $N\in\mathbb{Z}$), (see \cite{Das:2022slz}),
\begin{align}
    \chi^\mathcal{H}(\tau) = (j^{2+})^{\frac{N}{4}-s}\left[(j^{2+})^s + a_1\,(j^{2+})^{s-1}+ a_2 \, (j^{2+})^{s-2} + \ldots\ldots + a_s\right],
\label{gen_j}
\end{align}
where $s := \left \lfloor \frac{N}{4} \right \rfloor$.

\subsection{2-character MLDE}\label{sec2}
\subsubsection{$\ell=0$ analysis}
With the above derivative operator as defined in Eq.(\ref{deriv_op}) now let us set up the (2,0) MLDE,
\begin{align}
    \left(\Tilde{D}^2 + \mu_1E_4^{2+}\right)\chi = 0, \label{mlde20_0}
\end{align}
where $\chi$ is a weight 0 modular function for $\Gamma^{+}_0(2)$. Now substituting the Fourier expansions of the relevant terms in Eq.(\ref{mlde20_0}) we get the following recursion relation,
\begin{align}
    &\left[(\alpha+i)^2 - \frac{1}{4}(\alpha+i) + \mu_1\right]a_i = \sum\limits_{k=1}^i\left[\frac{1}{4}(\alpha+i-k)E^{2+}_{2,k}-\mu_1E_{4,k}^{2+}\right]a_{i-k}, \label{recursion0}
\end{align}
where $a_i$s are Fourier coefficients of the character $q$-series expansion.\\

The indicial equation is obtained by setting $i=0$ and $k=0$ in Eq.(\ref{recursion0}),
\begin{align}
    \alpha^2 - \frac{1}{4}\alpha + \mu_1 = 0. \label{indicial0}
\end{align}
Setting $\alpha=\alpha_0$ in Eq.(\ref{indicial0}) we get,
\begin{align}
    \mu_1 = \frac{1}{4}\left(\alpha_0-4\alpha_0^2\right), \label{param0}
\end{align}
Now setting $i=1$ in Eq.(\ref{recursion0}) we get the following quadratic equation in $\alpha_0$,
\begin{align}
    9a_1 + 168\alpha_0 + 24a_1\alpha_0 - 576\alpha_0^2 = 0, \label{m1_eqn_0}
\end{align}
which can be recast as below if we identify $N=-24\alpha_0=c$,
\begin{align}
    -9a_1 + 7N + a_1N + N^2 = 0, \label{N_eqn_0}
\end{align}
$a_1$ can now be expressed in terms of $N$ as,
\begin{align}
    a_1 = \frac{N(N+7)}{9-N}, \label{a1_eqn_0}
\end{align}
which sets an upper bound on the central charge $c<9$. Furthermore, applying the integer root theorem to Eq.(\ref{N_eqn_0}), we see that $c=N\in\mathbb{Z}$.
\\

Now checking for higher orders (upto $\mathcal{O}(q^{5000})$) for both characters, for $0<c<9$, we find the following admissible character solutions,
\begin{itemize}
    \item $(c,h)=\left(1,\frac{1}{3}\right)$: 
    \begin{align}
        &\chi_0 = q^{-1/24}(1 + q + 2q^2 + q^3 + 3q^4 + 3q^5 + 5q^6 + 5q^7 + 8q^8 + 8q^9 + 12q^{10} + \mathcal{O}(q^{11})), \nonumber\\
        &\chi_{\frac{1}{3}} = q^{7/24}(1 + q^2 + q^3 + 2q^4 + 1q^5 + 3q^6 + 2q^7 + 5q^8 + 4q^9 + 7q^{10} + \mathcal{O}(q^{11}))
    \end{align}
    \item $(c,h)=\left(3,\frac{1}{2}\right)$: 
    \begin{align}
        &\chi_0 = q^{-1/8}(1 + 5q + 11q^2 + 20q^3 + 41q^4 + 76q^5 + 127q^6 + 211q^7 + 342q^8 + 541q^9 + 838q^{10} + \mathcal{O}(q^{11})), \nonumber\\
        &\chi_{\frac{1}{2}} = q^{3/8}(1 + q + 5q^2 + 6q^3 + 16q^4 + 21q^5 + 46q^6 + 61q^7 + 117q^8 + 157q^{9} + 273 q^{10} +  \mathcal{O}(q^{11}))
    \end{align}
    \item $(c,h)=\left(5,\frac{2}{3}\right)$: 
    \begin{align}
        \chi_0 &= q^{-5/24}(1 + 15q + 40q^2 + 135q^3 + 290q^4 + 726q^5 + 1415q^6 + 3000q^7 + 5485q^8 \nonumber\\
        &+ 10565q^9 + 18407q^{10} + \mathcal{O}(q^{11})), \nonumber\\
        \chi_{\frac{2}{3}} &= q^{11/24}(5 + 11q + 55q^2 + 100q^3 + 290q^4 + 535q^5 + 1235q^6 \nonumber\\
        &+ 2160q^7 + 4400q^8 + 7465q^{9} + 13945q^{10} + \mathcal{O}(q^{11}))
    \end{align}
\end{itemize}

We also find a \textit{identity only} admissible solution, which only has a nice identity character but unstable non-trivial character. This is found at $(c,h)=\left(6,\frac{3}{4}\right)$.
\begin{align}
    \chi_0 &= q^{-1/4}(1 + 26q + 79q^2 + 326q^3 + 755q^4 + 2106q^5 + 4460q^6 + 10284q^7 \nonumber\\
    &+ 20165q^8 + 41640q^9 + 77352q^{10} + \mathcal{O}(q^{11}))
\end{align}

For $c=7,8$, both the characters are unstable and for $c=2,4$ there exists no $a_1\in\mathbb{Z}$ solutions to Eq.(\ref{N_eqn_0}). \\

Now let us observe the $c=6$, \textit{identity only} solution. It turns out $\chi_{0}^{c=6} = ({j^{2+}})^{\frac{1}{4}}$. So, a $(1,1)$ solution has appeared as a $(2,0)$ solution, a phenomenon which keeps happening in the $\text{SL}(2,\mathbb{Z})$ case. So, we can use this phenomena: \textit{$(j^{2+})^x$ where $x\in\{\frac{1}{4},\frac{1}{2},\frac{3}{4}\}$ will always appear as a particular solution to a $(n,l)$ MLDE}, to reduce the no. of parameters of the $(n,l)$ MLDE by one. \\

For $c=6$, $\mu_1 = -\frac{1}{8}$ (using Eq.(\ref{param0})). With this value of $\mu_1$, Eq.(\ref{j2+mlde}) should yield a solution $\chi=({j^{2+}})^{\frac{1}{4}}$. This would lead to the following relation (after substituting $\chi=({j^{2+}})^{\frac{1}{4}}$ in Eq.(\ref{j2+mlde})),
\begin{align}
    \frac{j^{2+}}{j^{2+}-256} = \frac{(E_4^{2+})^3}{(E_6^{2+})^2}. \label{re_F2_again}
\end{align}

\subsubsection{Bilinear pairs}
Let ${}^{(2)}\mathcal{W}_1$, ${}^{(2)}\mathcal{W}_3$ and ${}^{(2)}\mathcal{W}_5$ denote the $c\in\{1,2,5\}$ admissible character-like (2,0) solutions. Note that we have the following bilinear identities,
\begin{align}
    &(j^{2+})^{\frac{1}{4}} = \chi_0^{{}^{(2)}\mathcal{W}_1}\chi_0^{{}^{(2)}\mathcal{W}_5} + 2 \, \chi_{\frac{1}{3}}^{{}^{(2)}\mathcal{W}_1}\chi_{\frac{2}{3}}^{{}^{(2)}\mathcal{W}_5}, \label{bilin0} \\
    &(j^{2+})^{\frac{1}{4}} = \chi_0^{{}^{(2)}\mathcal{W}_3}\chi_0^{{}^{(2)}\mathcal{W}_3} + 16 \, \chi_{\frac{1}{2}}^{{}^{(2)}\mathcal{W}_3}\chi_{\frac{1}{2}}^{{}^{(2)}\mathcal{W}_3}, \label{bilin1}
\end{align}
where Eq.(\ref{bilin1}) is a self-dual relation and where the above bilinears are for the following relation: $(2,0)\overset{c^\mathcal{H}=6}{\underset{n_1=1}{\longleftrightarrow}}(2,0)$ (where $n_1=\text{sum of conformal dimensions of the bilinear pair}$).\\

These bilinear relations can probably help us to write down the modular invariant partition function for the $(2,0)$ admissible solutions. For instance the below could be true\footnote{\AD{Ask Sunil Sir about this..}},
\begin{align}
    &\mathcal{Z}_1 = \left|\chi_0^{{}^{(2)}\mathcal{W}_1}\right|^2 + 2 \, \left|\chi_{\frac{1}{3}}^{{}^{(2)}\mathcal{W}_1}\right|^2, \label{partintn1} \\
    &\mathcal{Z}_3 = \left|\chi_0^{{}^{(2)}\mathcal{W}_3}\right|^2 + 16 \, \left|\chi_{\frac{1}{2}}^{{}^{(2)}\mathcal{W}_3}\right|^2, \label{partintn3} \\
    &\mathcal{Z}_5 = \left|\chi_0^{{}^{(2)}\mathcal{W}_5}\right|^2 + 2 \, \left|\chi_{\frac{2}{3}}^{{}^{(2)}\mathcal{W}_5}\right|^2, \label{partintn5}
\end{align}

\subsubsection{$\ell=1$ analysis}
Now let us move onto $\ell=1$ case. The MLDE reads (with $\frac{k}{8}$ derivative operator),
\begin{align}
    &\left[\Tilde{D}^2+\left(\mu_1\frac{(E_4^{2+})^2}{E_6^{2+}}+\mu_2\frac{\Delta_2}{E_6^{2+}}\right)\Tilde{D}+\mu_3\frac{E_{10}^{2+}}{E_{6}^{2+}}\right]\chi = 0, \label{mldeF2_2char_l1} \\
    &\left[E_6^{2+}\Tilde{D}^2 + \left(\mu_1(E_4^{2+})^2 + \mu_2\Delta_2\right)\Tilde{D} + \mu_3E_{10}^{2+}\right]\chi = 0. \label{mldeF2_2char_l1_aliter} \\
    &\left[E_6^{2+}q^2\partial_{q}^2 + \left(E_6^{2+} - \frac{E_6^{2+}E_2^{2+}}{4} + \mu_1(E_4^{2+})^2 + \mu_2\Delta_2\right)q\partial_q\chi + \mu_3 E_{10}^{2+} \right]\chi = 0. \label{qmldeF2_2char_l1}
\end{align}
From above we obtain the following recursion relation,
\begin{align}
    &\sum\limits_{k=0}^i\left[E_{6,k}^{2+}(\alpha^j+i-k)(\alpha^j+i-k-1) + E_{6,k}^{2+}(\alpha^j+i-k)-\frac{E_{2,k}^{2+}E_{2,k}^{2+}}{4}(\alpha^j+i-k)\right. \nonumber\\ 
    &\left.\mu_1 (E_{4}^{2+})^2_{,k} (\alpha^j+i-k) + \mu_2\Delta_{2,k}(\alpha^j+i-k) + \mu_3 E_{10,k}\right]a^j_{i-k} = 0, \label{recursion_l1F2_2char}
\end{align}
which gives the following indicial equation,
\begin{align}
    \alpha^2 + \left(\mu_1-\frac{1}{4}\right)\alpha + \mu_3 = 0, \label{indicial_l1F2_2char}
\end{align}
From Riemann-Roch (sum of exponents $= 0$), we see that $\mu_1=\frac{1}{4}$.\\

Now let us determine the value of $\mu_2$ by transforming the $\tau$-MLDE in Eq.(\ref{mldeF2_2char_l1}) into the corresponding $j^{2+}$-MLDE (about $\tau=\rho_2$),
\begin{align}
    \left[(j^{2+})^2\partial_{j^{2+}}^2 + \frac{j^{2+}}{2}\partial_{j^{2+}} +  \frac{j^{2+}}{j^{2+}-256}\left(\frac{j^{2+}}{2}-(64+\mu_2)\right)\partial_{j^{2+}} + \frac{\mu_3 j^{2+}}{j^{2+}-256}\right]\chi = 0, \label{j2+mlde_p2_l1}
\end{align}
where we have set $\mu_1=\frac{1}{4}$ from the $\ell=1$ indicial equation (see Eq.(\ref{indicial_l1F2_2char})). Now, note that about $\tau=\rho_2$, we have, $\chi_0\sim (j^{2+})^x$ and $j^{2+}\to 0$, with $x=\frac{1}{4}$ for $\ell=1$ (see $1$-character solutions). So, substituting $\chi=(j^{2+})^x$ about $j^{2+}=0$, the $j^{2+}$-indicial equation (which is basically, coefficient of $(j^{2+})^x$ $=\left.0\right|_{j^{2+}=0}$) reads,
\begin{align}
    x\left(x+\frac{\mu_2}{256}-\frac{1}{4}\right) = 0, \label{jindip2l1F2}
\end{align}
which yields $\mu_2 = 0$ for $x=\frac{1}{4}$. \\

Putting $i=1$ in Eq.(\ref{recursion_l2F2_2char}) yields\footnote{We shall at times identify $m_i:=a^0_i$.},
\begin{align}
    &m_1 + 40 \alpha_0 + 2 m_1 \alpha_0 - 48 \alpha_0^2 = 0, \label{m1al1}\\
    &-12 m_1 + 20 N + m_1 N + N^2 = 0 \, \, \, \, (\text{where}, \ N:=-24\alpha_0 = c). \label{diophNl1p2}
\end{align}
Applying integer root theorem to Eq.(\ref{diophNl1p2}) we note that $N=c\in\mathbb{Z}$.\\

With the above definition of $\alpha_0$ we can now find $m_1$ in terms of $N$,
\begin{align}
    m_1 = \frac{N(N+20)}{12-N}, \label{m1N_p2F2l1}
\end{align}
which implies that $0<c< 12$. Scanning this space of $c$, we observe that there exists the following admissible solutions.
\begin{itemize}
    \item $(c,h)=\left(4,\frac{1}{3}\right)$: 
    \begin{align}
        \chi_0 &= q^{-1/6}(1 + 12q + 70q^2 + 1304q^3 + 45969q^4 + 2110036q^5 + 109853542q^6 \nonumber\\
        &+ 6204772264q^7 + 371363466708q^8 + \mathcal{O}(q^{9})), \\
        \chi_{\frac{1}{3}} &= q^{1/6}(1 - 4q - 86q^2 - 2712q^3 - 110221q^4 - 5321572q^5 - 285692130q^6 \nonumber\\
        &- 16484830680q^7 - 1002347627239q^8 - \mathcal{O}(q^{9})),
    \end{align}
    where $\chi_0$ can be interpreted as a $c=4$ single-character solution. Surprisingly, this single-character solution is not ``yet" any $(1,l)$ solution. Also, note that, $\chi_{\frac{1}{3}}$ is a quasi-character of type II (see \cite{Chandra:2018pjq}).
    \item $(c,h)=\left(6,\frac{1}{2}\right)$: 
    \begin{align}
        &\chi_0 = (j^{2+})^{\frac{1}{4}}, \\
        &\chi_{\frac{1}{2}} = \text{unstable} \nonumber
    \end{align}
\end{itemize}

Note that, we can make use of the fact that $(j^{2+})^x$ with $x\in\{\frac{1}{2},\frac{3}{4}\}$ can also appear as a solution to the above $(2,1)$ MLDE and hence we get for these values of $x$, $\mu_2=-64$ and $\mu_2=-128$ respectively. \\

For $\mu_2=-64$ we get from the $i=1$ equation: $(m_1+c)\left(1-\frac{c}{12}\right)=0$ which implies $c=12$. So, this choice of $\mu_2$ only leads to one unitary single-character solution: $(j^{2+})^{\frac{1}{2}}$. \\

For $\mu_2=-128$, we get from the $i=1$ equation: $m_1=\frac{N(N-44)}{12-N}$ which means the allowed range of central charge is, $12<c<45$ (where $N=-24\alpha_0$). Scanning this space of $c$, we only obtain $(j^{2+})^{\frac{3}{4}}$ and three type II quasi-character solutions for $c=20,28,44$. So, this value of $\mu_2$ has no admissible 2-character solutions.

\subsubsection{$\ell=2$ analysis}
Now let us move to $\ell=2$ case. The MLDE reads (with $\frac{k}{8}$ derivative operator),
\begin{align}
    &\left(\Tilde{D}^2+\mu_1\frac{E_6^{2+}}{E_4^{2+}}\Tilde{D}+\mu_2E_4^{2+}+\mu_3\frac{\Delta_2}{E_{4}^{2+}}\right)\chi = 0, \label{mldeF2_2char_l2} \\
    &\left(E_4^{2+}\Tilde{D}^2 + \mu_1E_6^{2+}\Tilde{D} + \mu_2(E_4^{2+})^2 + \mu_3\Delta_2\right)\chi = 0. \label{mldeF2_2char_l2_aliter} \\
    &\left[E_4^{2+}q^2\partial_{q}^2 + \left(E_4^{2+} - \frac{E_4^{2+}E_2^{2+}}{4} + \mu_1E_6^{2+}\right)q\partial_q\chi + \mu_2(E_4^{2+})^2 + \mu_3\Delta_2\right]\chi = 0. \label{qmldeF2_2char_l2}
\end{align}
From above we obtain the following recursion relation,
\begin{align}
    &\sum\limits_{k=0}^i\left[E_{4,k}^{2+}(\alpha^j+i-k)(\alpha^j+i-k-1) + E_{4,k}^{2+}(\alpha^j+i-k)-\frac{E_{4,k}^{2+}E_{2,k}^{2+}}{4}(\alpha^j+i-k)\right. \nonumber\\ 
    &\left.\mu_1E_{6,k}^{2+}(\alpha^j+i-k) + \mu_2(E_4^{2+})_{,k}^2 + \mu_3\Delta_{2,k}\right]a^j_{i-k} = 0, \label{recursion_l2F2_2char}
\end{align}
which gives the following indicial equation,
\begin{align}
    \alpha^2 + \left(\mu_1-\frac{1}{4}\right)\alpha + \mu_2 = 0, \label{indicial_l2F2_2char}
\end{align}
From Riemann-Roch (sum of exponents $= -\frac{1}{4}$), we see that $\mu_1=\frac{1}{2}$.\\

Now let us determine the value of $\mu_3$ by transforming the $\tau$-MLDE in Eq.(\ref{mldeF2_2char_l2}) into the corresponding $j^{2+}$-MLDE (about $\tau=\rho_2$),
\begin{align}
    \left[(j^{2+})^2\partial_{j^{2+}}^2 + \frac{j^{2+}}{j^{2+}-256}\left(\frac{3j}{4}-64\right)\partial_{j^{2+}} + \frac{\mu_2 j^{2+}}{j^{2+}-256} + \frac{\mu_3}{j^{2+}-256}\right]\chi = 0, \label{j2+mlde_p2_l2}
\end{align}
where we have set $\mu_1=\frac{1}{2}$ from the $\ell=2$ indicial equation (see Eq.(\ref{indicial_l2F2_2char})). Now, note that about $\tau=\rho_2$, we have, $\chi_0\sim (j^{2+})^x$ and $j^{2+}\to 0$, with $x=\frac{1}{2}$ for $\ell=2$ (see $1$-character solutions). So, substituting $\chi=(j^{2+})^x$ about $j^{2+}=0$, the $j^{2+}$-indicial equation (which is basically, coefficient of $(j^{2+})^x$ $=\left.0\right|_{j^{2+}=0}$) reads,
\begin{align}
    x^2-\frac{3}{4}x - \frac{\mu_3}{256} = 0, \label{jindip2l2F2}
\end{align}
which yields $\mu_3 = -32$ for $x=\frac{1}{2}$. Another root of the above equation with $\mu_3=-32$ is $x=\frac{1}{4}$. \\

Putting $i=1$ in Eq.(\ref{recursion_l2F2_2char}) yields\footnote{We shall at times identify $m_i:=a^0_i$.},
\begin{align}
    &-128 + 5 m_1 - 248 \alpha_0 + 8 m_1 \alpha_0 - 192 \alpha_0^2 = 0, \label{m1al}\\
    &384 - 15 m_1 - 31 N + m_1 N + N^2 = 0 \, \, \, \, (\text{where}, \ N:=-24\alpha_0 = c). \label{diophNl2p2}
\end{align}
Applying integer root theorem to Eq.(\ref{diophNl2p2}) we note that $N=c\in\mathbb{Z}$.\\

With the above definition of $\alpha_0$ we can now find $m_1$ in terms of $N$,
\begin{align}
    m_1 = (16-N)+\frac{144}{15-N}, \label{m1N_p2F2l2}
\end{align}
which implies that $0<c< 15$. Scanning this space of $c$, we observe that there exists the following admissible solutions.
\begin{itemize}
    \item $(c,h)=\left(3,0\right)$: 
    \begin{align}
        \chi_0 &= q^{-1/8}(1 + 25q + 51q^2 + 196q^3 + 297q^4 + 780q^5 + 1223q^6 \nonumber\\
        &+ 2551q^7 + 3798q^8 + 7201q^9 + 10582q^{10} + \mathcal{O}(q^{11})),
    \end{align}
    where since $h=0$ both the characters are identical. This is a $1$-character solution which surprisingly is not ``yet" any $(1,l)$ solution.
    \item $(c,h)=\left(6,\frac{1}{4}\right)$: 
    \begin{align}
        &\chi_0 = (j^{2+})^{\frac{1}{4}}, \\
        &\chi_{\frac{1}{4}} = \text{unstable} \nonumber
    \end{align}
    \item $(c,h)=\left(7,\frac{1}{3}\right)$: 
    \begin{align}
        &\chi_0 = (j^{2+})^{\frac{1}{4}}\otimes \chi_0^{{}^{(2)}\mathcal{W}_1} \nonumber\\
        &\chi_{\frac{1}{3}} = (j^{2+})^{\frac{1}{4}}\otimes \chi_{\frac{1}{3}}^{{}^{(2)}\mathcal{W}_1}
    \end{align}
    \item $(c,h)=\left(9,\frac{1}{2}\right)$: 
    \begin{align}
        &\chi_0 = (j^{2+})^{\frac{1}{2}}\otimes \chi_0^{{}^{(2)}\mathcal{W}_3} \nonumber\\
        &\chi_{\frac{1}{2}} = (j^{2+})^{\frac{1}{4}}\otimes \chi_{\frac{1}{2}}^{{}^{(2)}\mathcal{W}_3}
    \end{align}
    \item $(c,h)=\left(11,\frac{2}{3}\right)$: 
    \begin{align}
        &\chi_0 = (j^{2+})^{\frac{2}{3}}\otimes \chi_0^{{}^{(2)}\mathcal{W}_5} \nonumber\\
        &\chi_{\frac{2}{3}} = (j^{2+})^{\frac{1}{4}}\otimes \chi_{\frac{2}{3}}^{{}^{(2)}\mathcal{W}_5}
    \end{align}
    \item $(c,h)=\left(12,\frac{3}{4}\right)$: 
    \begin{align}
        &\chi_0 = (j^{2+})^{\frac{1}{2}}, \\
        &\chi_{\frac{3}{4}} = \text{unstable} \nonumber
    \end{align}
\end{itemize}
Let ${}^{(2)}\mathcal{W}_7$, ${}^{(2)}\mathcal{W}_9$ and ${}^{(2)}\mathcal{W}_{11}$ denote the $c\in\{7,9,11\}$ admissible character-like (2,2) solutions. Note that, here also, we have some bilinear identities,
\begin{align}
    &(j^{2+})^{\frac{3}{4}} = \chi_0^{{}^{(2)}\mathcal{W}_7}\chi_0^{{}^{(2)}\mathcal{W}_{11}} + 2 \, \chi_{\frac{1}{3}}^{{}^{(2)}\mathcal{W}_7}\chi_{\frac{2}{3}}^{{}^{(2)}\mathcal{W}_{11}}, \label{bilin2} \\
    &(j^{2+})^{\frac{1}{4}} = \chi_0^{{}^{(2)}\mathcal{W}_9}\chi_0^{{}^{(2)}\mathcal{W}_9} + 16 \, \chi_{\frac{1}{2}}^{{}^{(2)}\mathcal{W}_9}\chi_{\frac{1}{2}}^{{}^{(2)}\mathcal{W}_9}, \label{bilin3}
\end{align}
where Eq.(\ref{bilin3}) is a self-dual relation. Note, Eqs.(\ref{bilin2}) and (\ref{bilin3}) are nothing but $(j^{2+})^{\frac{1}{2}}$ multiplied with Eqs.(\ref{bilin0}) and (\ref{bilin1}) respectively. More bilinear pairs can be constructed by multiplying $(j^{2+})^{\frac{1}{4}}$ multiplied with Eqs.(\ref{bilin0}) and (\ref{bilin1}). \\

Note that, we can make use of the fact that $(j^{2+})^x$ with $x\in\{\frac{3}{4}\}$ can also appear as a solution to the above $(2,2)$ MLDE and hence we get for this value of $x$, $\mu_3=0$. \\

For $\mu_3=0$, we get from the $i=1$ equation: $m_1=\frac{N(N-31)}{15-N}$ where $N=-24\alpha_0$. This gives the allowed range of central charge as, $15<c<32$. Scanning this space of $c$ we get the following admissible solutions.

\begin{itemize}
    \item $(c,h)=\left(19,\frac{4}{3}\right)$: 
    \begin{align}
        \chi_0 &= q^{-19/24}(1 + 57q + 2147q^2 + 31540q^3 + 260243q^4 + 1691798q^5  \nonumber\\
        &+ 8887877q^6 + 41091167q^7 + 168938614q^8 + \mathcal{O}(q^{9})), \nonumber\\
        \chi_{\frac{4}{3}} &= q^{13/24}(133 + 2717q + 33839q^2 + 246468q^3 + 1506510q^4 + 7478629q^5 + 33354310q^6 \nonumber\\
        &+ 132591975q^7 + 489341675q^8 + \mathcal{O}(q^{9}))
    \end{align}
    \item $(c,h)=\left(21,\frac{3}{2}\right)$: 
    \begin{align}
        \chi_0 &= q^{-7/8}(1 + 35q + 2394q^2 + 40873q^3 + 405426q^4 + 2946132q^5  \nonumber\\
        &+ 17381133q^6 + 88016962q^7 + 395953299q^8 + \mathcal{O}(q^{9})), \nonumber\\
        \chi_{\frac{3}{2}} &= q^{5/8}(7 + 161q + 2160q^2 + 17409q^3 + 115003q^4 + 619101q^5 + 2962183q^6 \nonumber\\
        &+ 12628973q^7 + 49681296q^8 + \mathcal{O}(q^{9}))
    \end{align}
    \item $(c,h)=\left(23,\frac{5}{3}\right)$: 
    \begin{align}
        \chi_0 &= q^{-23/24}(1 + 23q + 3335q^2 + 67068q^3 + 793776q^4 + 6461689q^5  \nonumber\\
        &+ 42601060q^6 + 236116965q^7 + 1157910689q^8 + \mathcal{O}(q^{9})), \nonumber\\
        \chi_{\frac{5}{3}} &= q^{17/24}(506 + 12903q + 185725q^2 + 1639463q^3 + 11650696q^4 + 67590238q^5 + 345549517q^6 \nonumber\\
        &+ 1572505630q^7 + 6570405101q^8 + \mathcal{O}(q^{9}))
    \end{align}
\end{itemize}

For $\mu_3=-112$, we get from the $i=1$ equation: $m_1=\frac{N(N-10)}{18-N}$ where $N=-24\alpha_0$. This gives the allowed range of central charge as, $9<c<18$. Scanning this space of $c$ we find no admissible solutions. We did not get any quasi-character solutions also.

\subsubsection{Non-trivial bilinear pairs}
Let us give here some more bilinear pairs which are non-trivial in the sense that they cannot be derived from Eqs.(\ref{bilin0}) and (\ref{bilin1}). Let ${}^{(2)}\mathcal{W}_{19}$, ${}^{(2)}\mathcal{W}_{21}$ and ${}^{(2)}\mathcal{W}_{23}$ denote the $c\in\{19,21,23\}$ admissible character-like (2,2) solutions (obtained with $\mu_3=0$).
\begin{align}
    &j^{2+} - 32 = \chi_0^{{}^{(2)}\mathcal{W}_5}\chi_0^{{}^{(2)}\mathcal{W}_{19}} + 2 \, \chi_{\frac{2}{3}}^{{}^{(2)}\mathcal{W}_5}\chi_{\frac{4}{3}}^{{}^{(2)}\mathcal{W}_{19}}, \label{bilin_non_0} \\
    &j^{2+} - 64 = \chi_0^{{}^{(2)}\mathcal{W}_3}\chi_0^{{}^{(2)}\mathcal{W}_{21}} + 256 \, \chi_{\frac{1}{2}}^{{}^{(2)}\mathcal{W}_3}\chi_{\frac{3}{2}}^{{}^{(2)}\mathcal{W}_{21}}, \label{bilin_non_1} \\
    &j^{2+} - 80 = \chi_0^{{}^{(2)}\mathcal{W}_1}\chi_0^{{}^{(2)}\mathcal{W}_{23}} + 2 \, \chi_{\frac{1}{3}}^{{}^{(2)}\mathcal{W}_1}\chi_{\frac{5}{3}}^{{}^{(2)}\mathcal{W}_{23}}, \label{bilin_non_2}
\end{align}
where the above bilinears are for the following relation: $(2,0)\overset{c^\mathcal{H}=24}{\underset{n_1=2}{\longleftrightarrow}}(2,2)$. \\

Furthermore, we also have,
\begin{align}
    &(j^{2+})^{\frac{3}{4}}(j^{2+}-102) = \chi_0^{{}^{(2)}\mathcal{W}_{19}}\chi_0^{{}^{(2)}\mathcal{W}_{23}} + 2 \, \chi_{\frac{4}{3}}^{{}^{(2)}\mathcal{W}_{19}}\chi_{\frac{5}{3}}^{{}^{(2)}\mathcal{W}_{23}}, \label{bilin_non_3} \\
    &(j^{2+})^{\frac{3}{4}}(j^{2+}-112) = \chi_0^{{}^{(2)}\mathcal{W}_{21}}\chi_0^{{}^{(2)}\mathcal{W}_{21}} + 256 \, \chi_{\frac{3}{2}}^{{}^{(2)}\mathcal{W}_{21}}\chi_{\frac{3}{2}}^{{}^{(2)}\mathcal{W}_{21}}, \label{bilin_non_4} \\
\end{align}
where the above bilinears are for the following relation: $(2,2)\overset{c^\mathcal{H}=42}{\underset{n_1=3}{\longleftrightarrow}}(2,2)$.\footnote{A similar analysis should be performed with the $\frac{k}{12}$ derivative operator (the usual one)In this case, we can tune the $\mu_1$ parameter to even make this MLDE consistent with the Riemann-Roch. This is because in this case there exists a weight $2$ meromorphic form contribution to the MLDE due to the allowance of poles in the coefficient functions present in the MLDE.}.

\subsubsection{$\ell=3$ analysis}
Now let us move to the $\ell=3$ case. The MLDE reads (with $\frac{k}{8}$ derivative operator)\footnote{The generic form of the $(2,3)$ MLDE is exactly the same as the $(2,1)$ MLDE and only the values of the parameters in the MLDE will change.},
\begin{align}
    &\left[\Tilde{D}^2+\left(\mu_1\frac{(E_4^{2+})^2}{E_6^{2+}}+\mu_2\frac{\Delta_2}{E_6^{2+}}\right)\Tilde{D}+\mu_3\frac{E_{10}^{2+}}{E_{6}^{2+}}\right]\chi = 0, \label{mldeF2_2char_l3} \\
    &\left[E_6^{2+}\Tilde{D}^2 + \left(\mu_1(E_4^{2+})^2 + \mu_2\Delta_2\right)\Tilde{D} + \mu_3E_{10}^{2+}\right]\chi = 0. \label{mldeF2_2char_l3_aliter} \\
    &\left[E_6^{2+}q^2\partial_{q}^2 + \left(E_6^{2+} - \frac{E_6^{2+}E_2^{2+}}{4} + \mu_1(E_4^{2+})^2 + \mu_2\Delta_2\right)q\partial_q\chi + \mu_3 E_{10}^{2+} \right]\chi = 0. \label{qmldeF2_2char_l3}
\end{align}
From above we obtain the following recursion relation,
\begin{align}
    &\sum\limits_{k=0}^i\left[E_{6,k}^{2+}(\alpha^j+i-k)(\alpha^j+i-k-1) + E_{6,k}^{2+}(\alpha^j+i-k)-\frac{E_{2,k}^{2+}E_{2,k}^{2+}}{4}(\alpha^j+i-k)\right. \nonumber\\ 
    &\left.\mu_1 (E_{4}^{2+})^2_{,k} (\alpha^j+i-k) + \mu_2\Delta_{2,k}(\alpha^j+i-k) + \mu_3 E_{10,k}\right]a^j_{i-k} = 0, \label{recursion_l1F2_2char}
\end{align}
which gives the following indicial equation,
\begin{align}
    \alpha^2 + \left(\mu_1-\frac{1}{4}\right)\alpha + \mu_3 = 0, \label{indicial_l3F2_2char}
\end{align}
From Riemann-Roch (sum of exponents $= -\frac{1}{2}$), we see that $\mu_1=\frac{3}{4}$.
\\

Now let us determine the value of $\mu_2$ by transforming the $\tau$-MLDE in Eq.(\ref{mldeF2_2char_l3}) into the corresponding $j^{2+}$-MLDE (about $\tau=\rho_2$),
\begin{align}
    \left[(j^{2+})^2\partial_{j^{2+}}^2 + \frac{j^{2+}}{2}\partial_{j^{2+}} -  \frac{j^{2+}}{j^{2+}-256}\left((64+\mu_2)\right)\partial_{j^{2+}} + \frac{\mu_3 j^{2+}}{j^{2+}-256}\right]\chi = 0, \label{j2+mlde_p2_l3}
\end{align}
where we have set $\mu_1=\frac{3}{4}$ from the $\ell=3$ indicial equation (see Eq.(\ref{indicial_l3F2_2char})). Now, note that about $\tau=\rho_2$, we have, $\chi_0\sim (j^{2+})^x$ and $j^{2+}\to 0$, with $x=\frac{3}{4}$ for $\ell=3$ (see $1$-character solutions). So, substituting $\chi=(j^{2+})^x$ about $j^{2+}=0$, the $j^{2+}$-indicial equation (which is basically, coefficient of $(j^{2+})^x$ $=\left.0\right|_{j^{2+}=0}$) reads,
\begin{align}
    x^2-\frac{x}{2}+\frac{1}{4}+\frac{\mu_2}{256} = 0, \label{jindip2l3F2}
\end{align}
which yields $\mu_2 = -112$ for $x=\frac{3}{4}$. Similar analysis gives, $(x,\mu_2)=(\frac{1}{4},-48)$, $(x,\mu_2)=(\frac{1}{2},-64)$ as solution to Eq.(\ref{jindip2l3F2}).\\

For $\mu_2=-48$, we get from the $i=1$ equation: $m_1=\frac{N(N+22)}{18-N}$ where $N=-24\alpha_0$. This gives the allowed range of central charge as, $0<c<18$. Scanning this space of $c$ we get the following admissible solutions.

\begin{itemize}
    \item $(c,h)=\left(6,0\right)$: 
    \begin{align}
        \chi_0 &= q^{-1/4}(1 + 14q + 331q^2 + 4506q^3 + 112795q^4 + 3965662q^5  \nonumber\\
        & + 175520124q^6 + 8718679572q^7 + 470448806341q^8 + \mathcal{O}(q^{9})), \nonumber\\
        \chi_{\text{non-id}} &= \text{unstable}
    \end{align}
    where the above is a $1$-character solution (not yet a $(1,l)$ solution).
\end{itemize}

For $\mu_2=-64$, we get from the $i=1$ equation: $m_1=\frac{N(N+14)}{18-N}$ where $N=-24\alpha_0$. This gives the allowed range of central charge as, $0<c<18$. Scanning this space of $c$ we get the following admissible solutions.

\begin{itemize}
    \item $(c,h)=\left(6,0\right)$: 
    \begin{align}
        \chi_0 &= q^{-1/4}(1 + 10q + 367q^2 + 6422q^3 + 169555q^4 + 6322026q^5  \nonumber\\
        & + 286760396q^6 + 14591718924q^7 + 802225180229q^8 + \mathcal{O}(q^{9})), \nonumber\\
        \chi_{\text{non-id}} &= \text{unstable}
    \end{align}
    where the above is a $1$-character solution (not yet a $(1,l)$ solution).
    \item $(c,h)=\left(12,\frac{1}{2}\right)$: 
    \begin{align}
        \chi_0 &= (j^{2+})^{\frac{1}{2}}, \nonumber\\
        \chi_{\text{non-id}} &= 1
    \end{align}
\end{itemize}

\subsection{$j^{2+}$ analysis of $(2,0)$ solutions}
With Eqs.(\ref{j1_2}) and (\ref{j1_21}) we can recast the MLDE in Eq.(\ref{mlde20_0}) as,
\begin{align}
    \left[(j^{2+})^2\left(\frac{E_6^{2+}}{E_4^{2+}}\right)^2\partial^2_{j^{2+}} + \left(\frac{1}{2}j^{2+}\left(\frac{E_6^{2+}}{E_4^{2+}}\right)^2+\frac{3j^{2+}}{4}E_4^{2+}-64E_4^{2+}\right)\partial_{j^{2+}} + \mu_1E_4^{2+}\right]\chi = 0. \label{j2+mlde}
\end{align}
Now let us divide Eq.(\ref{j2+mlde}) by $E_4^{2+}$ and then use Eq.(\ref{re_F2}) to get (about $\tau=\rho_2$),
\begin{align}
    \left[j^{2+}\left(j^{2+}-256\right)\partial_{j^{2+}}^2 + \left(\frac{5j^{2+}}{4}-192\right)\partial_{j^{2+}} + \mu_1\right]\chi = 0, \label{j2+mlde_sim}
\end{align}
Define, $J := \frac{j^{2+}}{256}$. Then, Eq.(\ref{j2+mlde_sim}) becomes,
\begin{align}
    \left[J(J-1)\partial_J^2 + \frac{1}{4}\left(5J-3\right)\partial_J + \mu_1\right]\chi = 0. \label{J2+mlde}
\end{align}
Eq.(\ref{J2+mlde}) is an hypergeometric differential equation whose solution is (about $\tau=\rho_2$),
\begin{align}
    \chi(J) = a \, \, {}_2F_1\left(\alpha,\beta;\frac{3}{4};J\right) + b \, \, J^{1/4} {}_2F_1\left(\beta+\frac{1}{4},\alpha+\frac{1}{4};\frac{5}{4};J\right), \label{sonlF220}
\end{align}
where $\alpha+\beta=\frac{1}{4}$ and $\alpha\beta=\mu_1$. Furthermore, $a$ and $b$ are integration constants.

\subsection{(3,0) MLDE}
The recursion relation reads,
\begin{align}
    &\left[(\alpha^j+i)(\alpha^j+i-1)(\alpha^j+i-2) + 3(\alpha^j+i)(\alpha^j+i-1) + (\alpha^j+i)\right]a^j_i \nonumber\\ 
    &+ \sum\limits_{k=0}^i\left[-\frac{3}{4}E_{2,k}^{2+}a^j_{i-k}(\alpha^j+i-k)(\alpha^j+i-k-1) - \frac{3}{4}E_{2,k}^{2+}a^j_{i-k}(\alpha^j+i-k)\right. \nonumber\\
    &\left.- \frac{1}{32}E_{4,k}^{2+}a^j_{i-k}(\alpha^j+i-k) - \frac{3}{32}(E_{2}^{2+})^2_{,k}a^j_{i-k}(\alpha^j+i-k) + \mu_1E_{4,k}^{2+}a^j_{i-k}(\alpha^j+i-k) + \mu_2E_{6,k}^{2+}a^j_{i-k}\right] = 0. \label{recursion3_2}
\end{align}
From which the indicial equation reads,
\begin{align}
    \alpha^3 - \frac{3}{4}\alpha + \left(\mu_1-\frac{1}{8}\right)\alpha + \mu_2 = 0. \label{indicial3_2}
\end{align}
Also,
\begin{align}
&-40 m_1^2 + 15 m_1 m_1 - 820 m_1 \alpha_0 - 376 m_1^2 \alpha_0 + 1880 m_2 \alpha_0 + 18 m_1 m_2 \alpha_0 + 15840 \alpha_0^2 - 11064 m_1 \alpha_0^2 \nonumber\\
&- 1104 m_1^2 \alpha_0^2 + 3216 m_2 \alpha_0^2 - 206784 \alpha_0^3 - 27456 m_1 \alpha_0^3 - 768 m_1^2 \alpha_0^3 + 1536 m_2 \alpha_0^3 + 225792 \alpha_0^4 = 0.
\end{align}

The Diophantine equation reads,
\begin{align}
&-338829120 m_1^2 + 127060920 m_1 m_2 + 5906460 m_1 N + 2708328 m_1^2 N - 13541640 m_2 N \nonumber\\
&- 129654 m_1 m_2 N + 97020 N^2 - 67767 m_1 N^2 - 6762 m_1^2 N^2 + 19698 m_2 N^2 + 1077 N^3 \nonumber\\
&+ 143 m_1 N^3 + 4 m_1^2 N^3 - 8 m_2 N^3 + N^4 = 0, \label{Diop1_3_2}
\end{align}


\section{$\mathbf{\Gamma^{+}_0(3)}$}
\subsection{Riemann-Roch}
The valence formula for $\Gamma^{+}_0(3)$ reads \cite{2006math......7408M},
\begin{align}\label{valence_Fricke_3}
    \nu_{\infty}(f) + \frac{1}{2}\nu_{\tfrac{i}{\sqrt{3}}}(f) + \frac{1}{6}\nu_{\rho_{3}}(f) + \sum\limits_{\substack{p\in\Gamma_{0}^{+}(3)\backslash\mathbb{H}^{2}\\ p\neq \tfrac{i}{\sqrt{3}},\rho_{3}}}\nu_{p}(f) = \frac{k}{6},
\end{align}
where $\rho_2 := -\frac{1}{2}+\frac{i}{2\sqrt{3}}$ and $\frac{i}{\sqrt{3}}$ is the Fricke involution point. From Proposition 4.3 of \cite{2006math......7408M}, we note that $E^{3+}_4$ has a zero at $\tau=\rho_3$ of order $4$ and $E^{2+}_6$ has a zero at $\tau=\rho_3$ of order $3$ and a zero at $\tau=\frac{i}{\sqrt{3}}$ of order 1. Also, $E^{3+}_8$ has a zero at $\tau=\rho_3$ of order $2$.\\

The Riemann-Roch for $\Gamma^{+}_0(3)$ reads,
\begin{align}
    \sum_{i=0}^{n-1} \, \alpha_i = \frac{n(n-1)}{6} - \frac{\ell}{3}, \label{RR3}
\end{align}
where, $n$ is the number of linearly independent characters, $\alpha_i$s are exponents and $\ell$ is the wronskian index.

\subsection{The operator}
Consider the following transformations (where $\gamma\in\Gamma^{+}_0(3)$),
\begin{align}
    &3E_2(3\gamma\tau) = 3(c\tau+d)^2E_2(3\tau) + \frac{6c}{i\pi}(c\tau+d), \label{E22tau_3} \\
    &E_2(\gamma\tau) = (c\tau+d)^2E_2(\tau) + \frac{6c}{i\pi}(c\tau+d), \label{E2tau_3} \\
    \text{leading to,} \, \, &E_2^{3+}(\gamma\tau) = (c\tau+d)^2E_2^{3+}(\tau) + \frac{3c}{i\pi}(c\tau+d) \label{E22+tau_3}.
\end{align}
Eq.(\ref{E22+tau_3}) motivates us to define the following derivative operator in the space of $\Gamma^{+}_0(3)$, acting on weight $k$ forms,
\begin{align}
    \Tilde{D}_k := \Tilde{\partial}_\tau - \frac{k}{6}E_2^{3+}(\tau). \label{deriv_op3}
\end{align}
where $\Tilde{\partial}_\tau := \frac{1}{2i\pi}\partial_\tau = q\partial_q$.
\\

One can check that for any modular form in $\Gamma^{+}_0(3)$, $\Tilde{D}_k$ maps $k$ forms to $k+2$ forms. Now if we construct the MLDE in the space of $\Gamma^{+}_0(3)$ withe the above derivative operator then the MLDE will be consistent with the Riemann-Roch formula for $\Gamma^{+}_0(3)$. However, if we use the usual \textit{Serre-Ramanujan} derivative to write down the MLDE in $\Gamma^{+}_0(3)$ then the resulting MLDE will not be consistent with the Riemann-Roch formula for $\Gamma^{+}_0(3)$.\\

We note below some interesting properties of the above derivative operator,
\begin{align}
    &\left(\Tilde{\partial}_{\tau} - \frac{1}{8}E_2^{3+}\right)E_2^{3+} = -\frac{1}{6}E_4^{3+}, \label{De2_3} \\
    &\Tilde{D}E_4^{3+} = -\frac{2}{3}E_6^{3+}, \label{De4_3} \\
    &\Tilde{D}E_6^{3+} = -(E_4^{3+})^2 + 54\Delta_{3,8}, \label{De4_3} \\
    &\Tilde{D}\Delta_{3,8} = -\frac{1}{3}\Delta_{3,10}, \label{Ddel38} \\
    \text{also,} \, \, &\Delta_{3,10}E_4^{3+} = \Delta_{3,8}E_{6}^{3+}, \label{prod_eq} \\
    \text{also,} \, \, &(E_4^{3+})^3 - (E_6^{3+})^2 = 108\Delta_{3,8}E_4^{3+}, \label{prod_eq1}
\end{align}
where $\Delta_{3,8} = \frac{41}{1728}\left((E_4^{3+})^3-E_8^{3+}\right)$ and $\Delta_{3,10} = \frac{61}{432}\left(E_4^{3+}E_6^{3+}-E_{10}^{2+}\right)$. \\

Now let us define the ``Hauptmodul" for $\Gamma^{+}_0(3)$,
\begin{align}
    j^{3+} = \frac{(E_4^{3+})^2}{\Delta_{3,8}}, \label{def_H_3}
\end{align}
We also have,
\begin{align}
    &\frac{j^{3+}}{j^{3+}-108} = \frac{(E_4^{3+})^3}{(E_6^{3+})^2}. \label{j-rel-e4e6_F3}
\end{align}
The above relation also shows,
\begin{align}
    &\lim\limits_{\tau\to\frac{i}{\sqrt{3}}} j^{3+}(\tau) = 108, \label{j2_1_F3} \\
    &\lim\limits_{\tau\to\rho_3} j^{3+}(\tau) = 0, \label{j2_2_F3} \\
    &\lim\limits_{\tau\to i\infty} j^{3+}(\tau) = \infty, \label{j2_3_F3}
\end{align}
Now it is straightforward to show that,
\begin{align}
    &\Tilde{\partial}_\tau = -j^{3+}\frac{E_6^{3+}}{E_4^{3+}}\partial_{j^{3+}}, \label{j1_2_F3} \\
    &\Tilde{D}^2 = (j^{3+})^2\left(\frac{E_6^{3+}}{E_4^{3+}}\right)^2\partial_{j^{3+}}^2 + \left(\frac{E_4^{3+}}{2}+\frac{5}{6}\left(\frac{E_6^{3+}}{E_4^{3+}}\right)^2\right)j^{3+}\partial_{j^{3+}}. \label{j1_2_F3_1}
\end{align}

\subsection{$\mathbf{(1,\ell\neq 0)}$ MLDE}\label{sec1_F3}
Let us do here some $1$-character computations. From Riemann-Roch we get that $c=8l$.
\\

$\ell=0$ is trivial so let us start with $\ell=1$. For $\ell=1$, the RHS of Valence Formula reads $\frac{1}{3}$ (since $k=2l$ always). The MLDE takes the following form,
\begin{align}
    \left[\Tilde{D} + \mu_1\frac{E_4^{3+}E_6^{3+}}{(E_4^{3+})^2+\mu\Delta_{3,8}} + \mu_2\frac{\Delta_{3,10}}{(E_4^{3+})^2+\mu\Delta_{3,8}}\right]\chi = 0. \label{F3_l1_p1}
\end{align}
Now using the indicial equation we can set $\mu_1=\frac{1}{3}$. Now let us take a guess, $\chi=(j^{3+})^{\frac{1}{3}}$. One can readily check that this is a solution with $\mu_2=\frac{\mu}{3}$.\\

Now let us analyse $\ell=2$. The MLDE takes the following form,
\begin{align}
    &\left(\Tilde{D}+\mu_1\frac{E_6^{3+}}{E_4^{3+}}\right)\chi = 0, \label{1char_F3_l2} \\
    &\left(E_4^{3+}\Tilde{D}+\mu_1E_6^{3+}\right)\chi = 0. \label{1char_F3_l2_aliter}
\end{align}
Note that in above $\Tilde{D}=q\partial_q$. Also, the indicial equation ($\alpha_0+\mu_1=0$) dictates $\mu_1=\frac{2}{3}$.\\

Now let us take a guess, $\chi=(j^{3+})^{\frac{2}{3}}$. Then, $\Tilde{\partial}_\tau (j^{3+})^{\frac{2}{3}} = -\frac{2}{3}(j^{3+})^{\frac{2}{3}}\frac{E_6^{3+}}{E_4^{3+}}$. Note, that this $\chi$ indeed satisfies Eq.(\ref{1char_F3_l2}) with $\mu_1=\frac{2}{3}$.\\

Now let us analyse $\ell=3$. We see from the Riemann-Roch that this is the \textit{bulk-pole} MLDE. The MLDE takes the following form,
\begin{align}
    &\left(\Tilde{D}+\mu_1\frac{(E_4^{3+})^2}{E_6^{3+}} + \mu_2\frac{\Delta_{3,8}}{E_6^{3+}}\right)\chi = 0, \label{1char_F3_l3} \\
    &\left(E_6^{3+}\Tilde{D}+\mu_1(E_4^{3+})^2 + \mu_2\Delta_{3,8}\right)\chi = 0. \label{1char_F3_l3_aliter}
\end{align}
Note that in above $\Tilde{D}=q\partial_q$. Also, the indicial equation ($\alpha_0+\mu_1=0$) dictates $\mu_1=1$.\\

Now let us take a guess, $\chi=j^{3+}+\mathcal{N}$. Then, substituting this in the differential equation in Eq.(\ref{1char_F3_l3_aliter}) we get,
\begin{align}
    &\left(E_6^{3+}\Tilde{D}+\mu_1(E_4^{3+})^2 + \mu2\Delta_{3,8}\right)(j^{3+}+\mathcal{N}) = \Delta_{3,8}\left[(108+b+\mathcal{N})j^{3+}+\mathcal{N}b\right]
\end{align}
So, we see that $j^{3+}+\mathcal{N}$ is a solution to the above differential equation iff,
\begin{align}
    &b=0 \, \, \, \text{and} \, \, \, \mathcal{N} = -108 \longrightarrow  \text{soln.:} \, \, j^{3+}-108, \label{sol1} \\
    &b=-108 \, \, \, \text{and} \, \, \, \mathcal{N} = 0 \longrightarrow  \text{soln.:} \, \, j^{3+}, \label{sol2}
\end{align}
Note that, $j^{3+}-108$ has $m_1<0$ and hence is not an admissible solution. So, the only admissible solution is: $j^{3+}$ which happens when $b=-108$ and $\mathcal{N}=0$. 
\\

So, here we do not get $j^{3+}+\mathcal{N}$ as a solution to the \textit{bulk-pole} MLDE. This is different from the $\text{SL}(2,\mathbb{Z})$ and the $\Gamma^{+}_0(2)$ case and probably this happens because of the following reason. In both $\text{SL}(2,\mathbb{Z})$ and $\Gamma^{+}_0(2)$, the \textit{bulk-pole} MLDE ($\ell=6$ and $\ell=4$, respectively), the \textit{bulk-pole} appears in the denominator ($D^r = E_4^3+\mu\Delta$ and $D^r=(E_4^{2+})^2+\mu\Delta_2$, respectively) while in $\Gamma^{+}_0(3)$ the \textit{bulk-pole} appears in the numerator ($N^r=(E_4^{3+})^2+\mu\Delta_{3,8}$).


\subsection{2-character MLDE}
\subsubsection{$\ell=0$ analysis}
With the above derivative operator as defined in Eq.(\ref{deriv_op3}) now let us set up the (2,0) MLDE,
\begin{align}
    \left(\Tilde{D}^2 + \mu_1E_4^{3+}\right)\chi = 0, \label{mlde20_3}
\end{align}
where $\chi$ is a weight 0 modular function for $\Gamma^{+}_0(3)$. Now substituting the Fourier expansions of the relevant terms in Eq.(\ref{mlde20_3}) we get the following recursion relation,
\begin{align}
    &\left[(\alpha+i)^2 - \frac{1}{3}(\alpha+i) + \mu_1\right]a_i = \sum\limits_{k=1}^i\left[\frac{1}{3}(\alpha+i-k)E^{3+}_{2,k}-\mu_1E_{4,k}^{3+}\right]a_{i-k}, \label{recursion3}
\end{align}
where $a_i$s are Fourier coefficients of the character $q$-series expansion.\\

The indicial equation is obtained by setting $i=0$ and $k=0$ in Eq.(\ref{recursion3}),
\begin{align}
    \alpha^2 - \frac{1}{3}\alpha + \mu_1 = 0. \label{indicial3}
\end{align}
Setting $\alpha=\alpha_0$ in Eq.(\ref{indicial3}) we get,
\begin{align}
    \mu_1 = \frac{1}{3}\left(\alpha_0-3\alpha_0^2\right), \label{param3}
\end{align}
Now setting $i=1$ in Eq.(\ref{recursion_l2F3_2char}) we get the following quadratic equation in $\alpha_0$,
\begin{align}
    4a_1 + 60\alpha_0 + 12a_1\alpha_0 - 144\alpha_0^2 = 0, \label{m1_eqn_3_l2}
\end{align}
which can be recast as below if we identify $N=-12\alpha_0=c/2$,
\begin{align}
    -4a_1 + 5N + a_1N + N^2 = 0, \label{N_eqn_3}
\end{align}
$a_1$ can now be expressed in terms of $N$ as,
\begin{align}
    a_1 = \frac{N(N+5)}{4-N}, \label{a1_eqn_3}
\end{align}
which sets an upper bound on the central charge $c<8$. Furthermore, applying the integer root theorem to Eq.(\ref{N_eqn_0}), we see that $c=2N$ and the central charge in this case is restricted to be an even integer.
\\

Now checking for higher orders (upto $\mathcal{O}(q^{5000})$) for both characters, for $0<c<8$ (even $c$), we find the following admissible character solutions,
\begin{itemize}
    \item $(c,h)=\left(2,\frac{1}{2}\right)$: 
    \begin{align}
        &\chi_0 = q^{-1/12}(1 + 2q + 2q^2 + 4q^3 + 5q^4 + 6q^5 + 11q^6 + 14q^7 + 17q^8 + 24q^9 + 31q^{10} + \mathcal{O}(q^{11})), \nonumber\\
        &\chi_{\frac{1}{2}} = q^{5/12}(1 + q^2 + 2q^3 + 2q^4 + 2q^5 + 5q^6 + 4q^7 + 7q^8 + 10q^9 + 11q^{10} + \mathcal{O}(q^{11}))
    \end{align}
\end{itemize}

We also find a \textit{identity only} admissible solution, which only has a nice identity character but unstable non-trivial character. This is found at $(c,h)=\left(4,\frac{2}{3}\right)$.
\begin{align}
    \chi_0 &= q^{-1/6}(1 + 7q + 8q^2 + 22q^3 + 42q^4 + 63q^5 + 106q^6 + 190q^7 \nonumber\\
    &+ 267q^8 + 428q^9 + 652q^{10} + \mathcal{O}(q^{11}))
\end{align}

For $c=6$, both the characters are unstable.

\subsubsection{$\ell=1$ analysis}
The $\ell=1$ mlde takes the following form,
\begin{align}
    \left[((E_4^{3+})^2+\mu\Delta_{3,8})\Tilde{D}^2 + (\mu_1E_4^{3+}E_6^{3+}+\mu_2\Delta_{3,10})\Tilde{D} + \mu_3 (E_4^{3+})^3 + \mu_4\frac{(\Delta_{3,8})^2}{E_4^{3+}} + \mu_5\Delta_{3,8}E_4^{3+}\right]\chi = 0. \label{mlde_F3_p2_l1}
\end{align}

\subsubsection{$\ell=2$ analysis}
With the above derivative operator as defined in Eq.(\ref{deriv_op3}) now let us set up the (2,2) MLDE,
\begin{align}
    \left(\Tilde{D}^2 + \mu_1\frac{E_6^{3+}}{E_4^{3+}}\Tilde{D} + \mu_2E_4^{3+} + \mu_3\frac{\Delta_{3,8}}{E_4^{3+}}\right)\chi = 0, \label{mlde22_3}
\end{align}
where $\chi$ is a weight 0 modular function for $\Gamma^{+}_0(3)$. Now substituting the Fourier expansions of the relevant terms in Eq.(\ref{mlde22_3}) we get the following recursion relation,
\begin{align}
    &\sum\limits_{k=0}^i\left[E_{4,k}^{3+}(\alpha^j+i-k)(\alpha^j+i-k-1) + E_{4,k}^{3+}(\alpha^j+i-k)-\frac{E_{2,k}^{3+}E_{4,k}^{3+}}{3}(\alpha^j+i-k)\right. \nonumber\\ 
    &\left.\mu_1 E_{6,k}^{3+} (\alpha^j+i-k) + \mu_2(E_4^{3+})^2_{,k} + \mu_3\Delta_{3,8,k}\right]a^j_{i-k} = 0, \label{recursion_l2F3_2char}
\end{align}
where $a_i$s are Fourier coefficients of the character $q$-series expansion.\\

The indicial equation is obtained by setting $i=0$ and $k=0$ in Eq.(\ref{recursion_l2F3_2char}),
\begin{align}
    \alpha^2 + \left(\mu_1-\frac{1}{3}\right)\alpha + \mu_2 = 0. \label{indicial_l2F3_2char}
\end{align}
Setting $\alpha=\alpha_0$ in Eq.(\ref{indicial_l2F3_2char}) and observing the Riemann-Roch we get,
\begin{align}
    &\mu_1 = \frac{2}{3}, \label{param2_l2F3}\\
    &\mu_2 = -\left(\alpha_0^2-\frac{\alpha_0}{3}\right), \label{param3_l2F3}
\end{align}
Now let us determine the value of $\mu_3$ by transforming the $\tau$-MLDE in Eq.(\ref{mlde22_3}) into the corresponding $j^{3+}$-MLDE (about $\tau=\rho_3$),
\begin{align}
    \left[(j^{3+})^2\partial_{j^{3+}}^2 + \frac{j^{3+}}{6}\partial_{j^{3+}} +  \frac{(j^{3+})^2}{2(j^{3+}-108)}\partial_{j^{3+}} + \frac{\mu_2 j^{3+}}{j^{3+}-108} + \frac{\mu_3}{j^{3+}-108}\right]\chi = 0, \label{j3+mlde_p2_l2}
\end{align}
where we have set $\mu_1=\frac{2}{3}$ from the $\ell=2$ indicial equation (see Eq.(\ref{indicial_l2F3_2char})). Now, note that about $\tau=\rho_3$, we have, $\chi_0\sim (j^{3+})^x$ and $j^{3+}\to 0$, with $x=\frac{2}{3}$ for $\ell=2$ (see $1$-character solutions). So, substituting $\chi=(j^{3+})^x$ about $j^{3+}=0$, the $j^{3+}$-indicial equation (which is basically, coefficient of $(j^{3+})^x$ $=\left.0\right|_{j^{3+}=0}$) reads,
\begin{align}
    x^2-\frac{5}{6}x-\frac{\mu_3}{108} = 0, \label{jindip2l2F3}
\end{align}
which yields $\mu_2 = -12$ for $x=\frac{2}{3}$. Similar analysis gives, $(x,\mu_2)=(\frac{1}{3},-18)$ as solution to Eq.(\ref{jindip2l2F3}).\\

For $\mu_3=-12$, we get from the $i=1$ equation: $m_1=9-N$ where $N=-12\alpha_0$. This gives the allowed range of central charge as, $0<c<10$ with $c\in 2\mathbb{Z}$. Scanning this space of $c$ we get the following admissible solutions.

\begin{itemize}
    \item $(c,h)=\left(4,0\right)$: 
    \begin{align}
        &\chi_0 = q^{-1/6}(1 + 7q + 8q^2 + 22q^3 + 42q^4 + 63q^5 + 106q^6 + 190q^7 + 267q^8 + 428q^9 + 652q^{10} + \mathcal{O}(q^{11})), \nonumber\\
        &\chi_{\text{non-id}} = \chi_0
    \end{align}
    \item $(c,h)=\left(6,\frac{1}{6}\right)$: 
    \begin{align}
        \chi_0 &= q^{-1/4}(1 + 6q + 8q^3 + 18q^4 + 17q^6 + 54q^7 + \mathcal{O}(q^{9})), \nonumber\\
        \chi_{\frac{1}{6}} &= q^{-1/12}(1 + 8q + 17q^2 + 46q^3 + 98q^4 + 198q^5 + 371q^6 + 692q^7 + 1205q^8 + \mathcal{O}(q^{9}))
    \end{align}
\end{itemize}

For $\mu_3=-18$, we get from the $i=1$ equation: $m_1=\frac{N^2-17N+108}{8-N}$ where $N=-12\alpha_0$. This gives the allowed range of central charge as, $0<c<8$ with $c\in 2\mathbb{Z}$. Scanning this space of $c$ we get the following admissible solutions.

\begin{itemize}
    \item $(c,h)=\left(4,0\right)$: 
    \begin{align}
        &\chi_0 = q^{-1/6}(1 + 13q + 50q^2 + 76q^3 + 222q^4 + 405q^5 + 664q^6 + 1222q^7 + 2121q^8 + 3146q^9 + + \mathcal{O}(q^{10})), \nonumber\\
        &\chi_{\text{non-id}} = \chi_0
    \end{align}
    \item $(c,h)=\left(8,\frac{1}{3}\right)$: 
    \begin{align}
        &\chi_0 = q^{-1/3}(1 + 14q + 65q^2 + 156q^3 + 456q^4 + 1066q^5 + 2250q^6 + 4720q^7 + 9426q^8 + 17590q^9 + \mathcal{O}(q^{10})), \nonumber\\
        &\chi_{\frac{1}{3}} = \text{unstable}
    \end{align}
    \item $(c,h)=\left(10,\frac{1}{2}\right)$: 
    \begin{align}
        &\chi_0 = (j^{3+})^{\frac{1}{3}}\otimes \chi_0^{{}^{(3)}\mathcal{W}_2} \nonumber\\
        &\chi_{\frac{1}{2}} = (j^{3+})^{\frac{1}{3}}\otimes \chi_{\frac{1}{2}}^{{}^{(3)}\mathcal{W}_2}
    \end{align}
    \item $(c,h)=\left(12,\frac{2}{3}\right)$: 
    \begin{align}
        &\chi_0 = q^{-2/3}(1 + 21q + 171q^2 + 745q^3 + 2418q^4 + 7587q^5 + 20510q^6 + 51351q^7 + \mathcal{O}(q^{8})), \nonumber\\
        &\chi_{\frac{2}{3}} = \text{unstable}
    \end{align}
\end{itemize}

\subsection{$j^{3+}$ analysis of $(2,0)$ solutions}
With Eqs.(\ref{j1_2_F3}) and (\ref{j1_2_F3_1}) we can recast the MLDE in Eq.(\ref{mlde20_3}) as,
\begin{align}
    \left[(j^{3+})^2\left(\frac{E_6^{3+}}{E_4^{3+}}\right)^2\partial^2_{j^{3+}} + \left(\frac{5}{6}j^{3+}\left(\frac{E_6^{3+}}{E_4^{3+}}\right)^2+\frac{j^{3+}E_4^{3+}}{2}\right)\partial_{j^{3+}} + \mu_1E_4^{3+}\right]\chi = 0. \label{j3+mlde}
\end{align}
Now let us divide Eq.(\ref{j3+mlde}) by $E_4^{3+}$ and then use Eq.(\ref{j-rel-e4e6_F3}) to get (about $\tau=\rho_3$),
\begin{align}
    \left[j^{3+}\left(j^{3+}-108\right)\partial_{j^{3+}}^2 + \left(\frac{5(j^{3+}-108)}{6}+\frac{j^{3+}}{2}\right)\partial_{j^{3+}} + \mu_1\right]\chi = 0, \label{j3+mlde_sim}
\end{align}
Define, $J := \frac{j^{3+}}{108}$. Then, Eq.(\ref{j3+mlde_sim}) becomes,
\begin{align}
    \left[J(J-1)\partial_J^2 + \frac{1}{6}\left(8J - 5\right)\partial_J + \mu_1\right]\chi = 0. \label{J3+mlde}
\end{align}
Eq.(\ref{J3+mlde}) is an hypergeometric differential equation whose solution is (about $\tau=\rho_3$),
\begin{align}
    \chi(J) = a \, \, {}_2F_1\left(\alpha,\beta;\frac{5}{6};J\right) + b \, \, J^{1/6} {}_2F_1\left(\beta+\frac{1}{6},\alpha+\frac{1}{6};\frac{7}{6};J\right), \label{sonlF320}
\end{align}
where $\alpha+\beta=\frac{1}{3}$ and $\alpha\beta=\mu_1$. Furthermore, $a$ and $b$ are integration constants.

\subsection{(3,0) MLDE}


\section{$\mathbf{\Gamma^{+}_0(5)}$}

\subsection{Riemann-Roch}
The Riemann-Roch for $\Gamma^{+}_0(5)$ reads,
\begin{align}
    \sum_{i=0}^{n-1} \, \alpha_i = \frac{n(n-1)}{4} - \frac{\ell}{2}, \label{RR5}
\end{align}
where, $n$ is the number of linearly independent characters, $\alpha_i$s are exponents and $\ell$ is the wronskian index.

\subsection{The operator}
Consider the following transformations (where $\gamma\in\Gamma^{+}_0(5)$),
\begin{align}
    &5E_2(5\gamma\tau) = 2(c\tau+d)^5E_2(5\tau) + \frac{6c}{i\pi}(c\tau+d), \label{E22tau5} \\
    &E_2(\gamma\tau) = (c\tau+d)^2E_2(\tau) + \frac{6c}{i\pi}(c\tau+d), \label{E2tau5} \\
    \text{leading to,} \, \, &E_2^{5+}(\gamma\tau) = (c\tau+d)^2E_2^{2+}(\tau) + \frac{2c}{i\pi}(c\tau+d) \label{E22+tau5}.
\end{align}
Eq.(\ref{E22+tau5}) motivates us to define the following derivative operator in the space of $\Gamma^{+}_0(5)$, acting on weight $k$ forms,
\begin{align}
    \Tilde{D}_k := \Tilde{\partial}_\tau - \frac{k}{4}E_2^{5+}(\tau). \label{deriv_op5}
\end{align}
where $\Tilde{\partial}_\tau := \frac{1}{2i\pi}\partial_\tau = q\partial_q$.
\\

One can check that for any modular form in $\Gamma^{+}_0(5)$, $\Tilde{D}_k$ maps $k$ forms to $k+2$ forms. Now if we construct the MLDE in the space of $\Gamma^{+}_0(5)$ withe the above derivative operator then the MLDE will be consistent with the Riemann-Roch formula for $\Gamma^{+}_0(5)$. However, if we use the usual \textit{Serre-Ramanujan} derivative to write down the MLDE in $\Gamma^{+}_0(5)$ then the resulting MLDE will not be consistent with the Riemann-Roch formula for $\Gamma^{+}_0(5)$.\\

We note below some interesting properties of the above derivative operator,
\begin{align}
    &\left(\Tilde{\partial}_{\tau} - \frac{1}{4}E_2^{5+}\right)E_2^{5+} = -\frac{1}{4}E_4^{5+} + \frac{4}{13}\Delta_5, \label{De25} \\
    &\Tilde{D}E_4^{5+} = -E_6^{5+}, \label{De45} \\
    &\Tilde{\partial}_\tau \Delta_5 = E_2^{5+}\Delta_5, \label{DeDel5} \\
    &\Tilde{D}\Tilde{E}_4^{5+} = -E_6^{5+}, \label{De45} \\
    &\Tilde{D}E_6^{5+} = -\frac{3}{2}E_8^{5+} - \frac{3224}{2817}\Delta_5E_4^{5+} + \frac{29000}{2817}\Delta_5 \Tilde{E}_4^{5+}, \label{De65} \\
    &\Tilde{D}E_6^{5+} = -\frac{3}{2}(E_4^{5+})^2 + \frac{464}{13}\Delta_5E_4^{5+} + \frac{20000}{169}\Delta_5^2, \label{De65_simp}, \\
    &\Tilde{D}E_6^{5+} = -\frac{3}{2}(\Tilde{E}_4^{5+})^2 + 44\Delta_5 \Tilde{E}_4^{5+} + 8\Delta_5^2, \label{De65_simp_E45p} \\
    &\frac{(E_6^{5+})^2}{(\Tilde{E}_4^{5+})^3} = -\frac{16}{(j^{5+})^2} - \frac{44}{j^{5+}} + 1 = \frac{(j^{5+}-x_1)(j^{5+}-x_2)}{(j^{5+})^2}. \label{e63-e42}
\end{align}
where $\Delta_5(\tau)=(\eta(\tau)\eta(5\tau))^4$ and $j^{5+}=\frac{\Tilde{E}_4^{5+}}{\Delta_5}$. Also, $\Tilde{E}_4^{5+} := (E_{2,5^{'}})^2$. We also note, $\Delta_5=\frac{13}{36}(\Tilde{E}_4^{5+}- E_4^{5+})$ and $E_8^{5+} = (E_4^{5+})^2 + \frac{16000}{4069}\Delta_5 E_4^{5+} - \frac{88000}{4069}\Delta_5 \Tilde{E}_4^{5+}$. We used these equations to re-write Eq.(\ref{De65}) as Eq.(\ref{De65_simp}). Also, $x_1=2(11-5\sqrt{5})$ and $x_2=2(11+5\sqrt{5})$.\\

Now it is straightforward to show that,
\begin{align}
    &\Tilde{\partial}_\tau = -j^{5+}\frac{E_6^{5+}}{\Tilde{E}_4^{5+}}\partial_{j^{5+}}, \label{j1_2_F5} \\
    &\Tilde{D}^2 = (j^{5+})^2\left(\frac{E_6^{5+}}{\Tilde{E}_4^{5+}}\right)^2\partial_{j^{5+}}^2 + \left(\frac{3}{2}\Tilde{E}_4^{5+} - 44\Delta_5 - 8\frac{\Delta_5^2}{\Tilde{E}_4^{5+}}\right)j^{5+}\partial_{j^{5+}}. \label{j1_2_F5_1}
\end{align}

\subsection{(2,0) MLDE}
With the above derivative operator as defined in Eq.(\ref{deriv_op}) now let us set up the (2,0) MLDE (note, $\Gamma^{+}_0(5)$ has a $2$-dimensional space of weight $4$ modular forms),
\begin{align}
    \left(\Tilde{D}^2 + \mu_1E_4^{5+} + \mu_2\Delta_5\right)\chi = 0, \label{mlde20_5}
\end{align}
where $\chi$ is a weight 0 modular function for $\Gamma^{+}_0(5)$. Now substituting the Fourier expansions of the relevant terms in Eq.(\ref{mlde20_5}) we get the following recursion relation,
\begin{align}
    &\left[(\alpha+i)^2 - \frac{1}{2}(\alpha+i) + \mu_1\right]a_i = \sum\limits_{k=1}^i\left[\frac{1}{2}(\alpha+i-k)E^{5+}_{2,k}-\mu_1 E_{4,k}^{5+} - \mu_2\Delta_{5,k}\right]a_{i-k}, \label{recursion05}
\end{align}
where $a_i$s are Fourier coefficients of the character $q$-series expansion.\\

The indicial equation is obtained by setting $i=0$ and $k=0$ in Eq.(\ref{recursion05}),
\begin{align}
    \alpha^2 - \frac{1}{2}\alpha + \mu_1 = 0. \label{indicial5}
\end{align}

We can try to do a $j^{5+}$ analysis to determine $\mu_2$. We can recast the MLDE in Eq.(\ref{mlde20_5}) in the $j^{5+}$ plane as follows,
\begin{align}
    \partial^2_{j^{5+}}\chi + \frac{3}{2}\frac{\left(j^{5+}-y_1\right)\left(j^{5+}-y_2\right)}{j^{5+}(j^{5+}-x_1)(j^{5+}-x_2)}\partial_{j^{5+}} + \frac{\mu_1 j^{5+} + \mu_2}{j^{5+}(j^{5+}-x_1)(j^{5+}-x_2)} = 0, \label{j5+20_F5}
\end{align}
where $y_1=\frac{4}{3}(11-2\sqrt{31})$, $y_2=\frac{4}{3}(11+2\sqrt{31})$, $x_1=2(11-5\sqrt{5})$ and $x_2=2(11+5\sqrt{5})$. The above differential equation is a Heun differential equation with the general solution being,
\begin{align}
    \chi &= a \, \text{HeunG}\left[-\frac{1}{2}\left(\frac{11x_2}{2}+2\right),\frac{\mu_2 x_2}{16},\frac{1}{4}(1-\sqrt{1-16\mu_1}),\frac{1}{4}(1+\sqrt{1-16\mu_1}),\frac{1}{2},\frac{1}{2},-\frac{j^{5+}x_2}{16}\right] \nonumber\\
    &+ \, b \, \sqrt{\frac{j^{5+}}{x_1}}\text{HeunG}\left[-\frac{1}{2}\left(\frac{11x_2}{2}+2\right),\frac{(\mu_2-11) x_2}{16},\frac{1}{4}(3+\sqrt{1-16\mu_1}),\frac{1}{4}(3-\sqrt{1-16\mu_1}),\frac{3}{2},\frac{1}{2},-\frac{j^{5+}x_2}{16}\right].
\end{align}


%
%==========================
  
    
    %%% Local Variables:
    %%% mode: latex
    %%% TeX-master: t
    %%% End:
 


==> MLDE_Hecke.tex <==
\section{Two-character MLDEs for Hecke groups}\label{sec:Hecke_MLDE}
\noindent There are certain subtleties we need to be careful of when formulating the covariant derivative that acts on modular forms belonging to Hecke groups. The key difference is that, unlike Fricke groups, Hecke groups possess non-zero dimensional space of weight $2$ modular forms. Thanks to this we don't need to include a quasi-modular form in the covariant derivative to preserve mapping from weight $r$ to weight $r+2$ forms. This being said, we could also define the covariant derivatives with the Eisenstein series of weight $2$ associated with the cusps to act as the quasi-modular forms. A distinct difference between Fricke and Hecke groups is that the latter possess a cusp at $\tau = 0$ in addition to others listed in table \ref{tab: Hecke_cusp_list}.
\\
\begin{table}[htb!]
    \centering
    \begin{tabular}{||c|c|c|c|c|c|c|c|c|c|c|c|c||}
     \hline
      $N$ & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 \\[0.5ex]
      \hline\hline
      $\tau$  & - & - & $-\tfrac{1}{2}$ & - & $-\tfrac{1}{2}$, $-\tfrac{1}{3}$ & - & $-\tfrac{1}{2}$, $-\tfrac{1}{4}$ & $-\tfrac{1}{3}$, $-\tfrac{1}{3}$ & $-\tfrac{1}{2}$, $-\tfrac{1}{5}$ & - & $-\tfrac{1}{2}$, $-\tfrac{1}{3}$, $-\tfrac{1}{4}$, $-\tfrac{1}{6}$\\[1ex]
    \hline
    \end{tabular}
    \caption{The non-trivial cusps of Hecke groups $\Gamma_{0}(N)$ apart from the ones at $\tau = 0,i\infty$ that is common to all levels.}
    \label{tab:  Hecke_cusp_list}
\end{table}
\\
Hence, the first choice for a Ramanujan-Serre covariant derivative for $\Gamma_{0}(N)$ is one that includes the Eisenstein series associated with the cusp at $\tau = 0$. Let us make the following definition
\begin{align}
    \begin{split}
        \mathcal{D} \equiv& \frac{1}{2\pi i}\frac{d}{d\tau} - \upsilon(r) E^{0}_{2,N}(\tau),\\
        \mathcal{D}^{n} =& \mathcal{D}_{r+2n-2}\circ\ldots\circ\mathcal{D}_{r+2}\circ\mathcal{D}_{r},
    \end{split}
\end{align}
where the Eisenstein series $E_{k,N}^{0}(\tau)$ is defined as follows \cite{Junichi}
\begin{align}
    E^{0}_{k,N}(\tau) = \begin{cases}
    -2^{\tfrac{k}{2} - \left\lfloor\left.\tfrac{N}{4}\right\rfloor\right.\tfrac{k}{2}}\frac{\left(E_{k}(2\tau) - E_{k}(\tau)\right)}{2^{k} - 1},\ &N = 2,4,8,\\
    \frac{-N^{\tfrac{k}{2}}\left(E_{k}(N\tau) - E_{k}(\tau)\right)}{N^{k} - 1},\ &N\in\mathbb{P},\\
    \frac{6^{\tfrac{k}{2}}\left(E_{k}(6\tau) - (3\tau) - E_{k}(2\tau) + E_{k}(\tau)\right)}{(3^{k} - 1)(2^{k} - 1)},\ &N = 6,\\
    \frac{10^{\tfrac{k}{2}}\left(E_{k}(10\tau) - E_{k}(5\tau) - E_{k}(2\tau) + E_{k}(\tau)\right)}{(5^{k} - 1)(2^{k} - 1)},\ &N = 10,\\
    2^{-\tfrac{k}{2}}E^{0}_{k,6}(\tau),\ &N = 12,\\
    \end{cases}
\end{align}
Another definition of the Ramanujan-Serre covariant derivatives in the $\Gamma_{0}(N)$ is one including the Eisenstein series associated with the cusp at $\tau = i\infty$ as follows
\begin{align}
    \begin{split}
        \mathcal{D} \equiv& \frac{1}{2\pi i}\frac{d}{d\tau} - \upsilon(r) E^{\infty}_{2,N}(\tau),\\
        \mathcal{D}^{n} =& \mathcal{D}_{r+2n-2}\circ\ldots\circ\mathcal{D}_{r+2}\circ\mathcal{D}_{r},
    \end{split}
\end{align}
where $E^{\infty}_{k,N}(\tau)$ is the Eisenstein series associated with the cusp $\infty$ is defined as follows \cite{Junichi}
\begin{align}
    E^{\infty}_{k,N}(\tau) = \begin{cases}
    \frac{2^{k}E_{k}(N\tau) - E_{k}\left(\tfrac{N\tau}{2}\right)}{2^{k} - 1},\ &N = 2,4,8,\\
    \frac{N^{k}E_{k}(N\tau) - E_{k}(\tau)}{N^{k} - 1},\ &N\in\mathbb{P},\\
    \frac{6^{k}E_{k}(6\tau) - 3^{k}(3\tau) - 2^{k}E_{k}(2\tau) + E_{k}(\tau)}{(3^{k} - 1)(2^{k} - 1)},\ &N = 6,\\
    \frac{10^{k}E_{k}(10\tau) - 5^{k}E_{k}(5\tau) - 2^{k}E_{k}(2\tau) + E_{k}(\tau)}{(5^{k} - 1)(2^{k} - 1)},\ &N = 10,\\
    E^{\infty}_{k,6}(2\tau),\ &N = 12,\\
    \end{cases}
\end{align}
for $k\geq 4$. The values of $\upsilon(r)$ for levels $N\leq 12$ and prime divisor levels of $\mathbb{M}$ $N>12$ are tabulated in \ref{tab:Hecke_valence}.
\begin{table}[htb!]
    \centering
    \begin{tabular}{||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c||}
    \hline
    $N$ & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11 & 12 & 13 & 17 & 19 & 23 & 29 & 31 & 41 & 59 & 71\\ [0.5ex]
    \hline\hline
    $\upsilon(r)$ & $\tfrac{r}{4}$ & $\tfrac{r}{3}$ & $\tfrac{r}{2}$ & $\tfrac{r}{2}$ & $r$ & $\tfrac{2r}{3}$ & $r$ & $r$ & $\tfrac{3r}{2}$ & $r$ & $2r$ & $\tfrac{7r}{6}$ & $\tfrac{3r}{2}$ & $\tfrac{5r}{2}$ & $2r$ & $\tfrac{5r}{2}$ & $\tfrac{8r}{3}$ & $\tfrac{7r}{2}$ & $5r$ & $6r$\\ [1ex]
    \hline
    \end{tabular}
    \caption{Values of $\upsilon(r) = \tfrac{r\overline{\mu}_{0}}{12}$ computed index data in table \ref{tab:Hecke_index_data}.}
    \label{tab:Hecke_valence}
\end{table}
\\
At level $N = 4$, we see from table \ref{tab:  Hecke_cusp_list} that the fundamental domain has a cusp at $\tau = -\tfrac{1}{2}$ and there exists an Eisenstein series associated with this cusp using which we can define yet another Ramanujan-Serre covariant derivative. Thus, we would have four unique MLDEs at level $N = 4$ and similarly, five unique MLDEs at levels $N = 6,8,9,10$, and seven unique MLDEs at level $N = 12$. The definitions of the Eisenstein series associated with the non-trivial cusps can be found in \cite{Junichi}.


==> Mathematical_preliminaries.tex <==
\section{Mathematical preliminaries}\label{appendix:A}
\subsection*{Definitions}
The special linear group over the integers $\text{SL}(2,\mathbb{Z})$ is defined as the set of all $2\times 2$ matrices with real entries and unit determinant, i.e.
\begin{equation}
    \text{SL}(2,\mathbb{Z}) = \left\{\left.\begin{pmatrix}
    a & b\\ c& d
    \end{pmatrix}\right\vert a,b,c,d\in\mathbb{R},ad-bc=1\right\}.
\end{equation}
The projective special linear group  over the integers or the modular group $\text{PSL}(2,\mathbb{Z})$ is nothing but the special linear group quotiented by $\mathbb{Z}_{2}$, i.e.
\begin{equation}
    \text{PSL}(2,\mathbb{Z}) = \text{SL}(2,\mathbb{Z})/\mathbb{Z}_{2} = \left\{\left.\begin{pmatrix}
    a & b\\ c& d
    \end{pmatrix}\right\vert a,b,c,d\in\mathbb{R},ad-bc=1\right\}/\{\pm 1\}.
\end{equation}
Since $\text{PSL}(2,\mathbb{Z})$ and $\text{SL}(2,\mathbb{Z})$ are equal up to a quotient $\mathbb{Z}_{2}$, both can be loosely referred to as the modular group. $\text{GL}(2,\mathbb{R})$ is the general linear group over the reals and is the group of all $2\times 2$ invertible matrices with coefficients in the ring $\mathbb{R}$ with $\text{SL}(2,\mathbb{R})$ being its subgroup with unit determinant. Let $\reallywidehat{\mathbb{C}} \equiv \mathbb{C}\cup \{\infty\}$ denote the Riemann sphere, which is also sometimes denoted by $\mathbb{P}^{1}(\mathbb{C})$. Let us consider an element $A\in\text{SL}(2,\mathbb{Z})$, where our ring now is the integers and the element $A$ is a $2\times 2$ matrix of the form
\begin{equation}
    A = \begin{pmatrix}
    a & b\\ c & d
    \end{pmatrix}.
\end{equation}
The action of $A$ on $\reallywidehat{\mathbb{C}}$ is defined by M\"obius or fractional linear transformations in the usual way
\begin{equation}
  A(z)\equiv \frac{az + b}{cz + d},
\end{equation}
and
\begin{align}\label{action_SL2Z}
\begin{split}
    A(\infty) = \lim\limits_{y\to \infty}\frac{a(x+iy) + b}{c(x+iy) + d} = \begin{cases}
    \frac{a}{c},\ &c\neq 0\\
    0,\ &c=0
    \end{cases}
\end{split}
\end{align}
The modular group contains the following three matrices
\begin{equation}
    I = \mathbb{1}_2,\ S = \begin{pmatrix}
    0 & -1\\ 1 & 0
    \end{pmatrix},\ T = \begin{pmatrix}
    1 & 1\\ 0 & 1
    \end{pmatrix},
\end{equation}
where $\mathbb{1}_{2}$ is the $2\times 2$ identity matrix. It is to be noted that different definitions are followed for the $S$ matrix with the convention of placing the $-1$ in different off-diagonal positions. We either denote $\left(\begin{smallmatrix}0 &-1\\ 1&\ 0\end{smallmatrix}\right)$ or $\left(\begin{smallmatrix}\ 0 &1\\ -1&0\end{smallmatrix}\right)$ to be the $S$ matrix and we shall stick to the former in this paper. The $S$ and the $T$ matrices generate the modular group. The discrete subgroups of $\text{PSL}(2,\mathbb{R})$ are denoted by $\overline{\Gamma}$ with the convention that we denote $\overline{\Gamma}(1) = \text{PSL}(2,\mathbb{Z})$ and the discrete subgroups of $\text{SL}(2,\mathbb{Z})$ are denoted by $\Gamma$ with the convention that $\Gamma(1) = \text{SL}(2,\mathbb{Z})$. These subgroups are related as $\overline{\Gamma} = \Gamma/\pm I$. The discrete subgroup of level $2$, for example, is defined as follows 
\begin{align}
    \begin{split}
    \Gamma(2) =& \left\{A\in\text{SL}(2,\mathbb{Z})\vert A\equiv \mathbb{1}_{2}\ (\text{mod}\ 2)\right\}\\
    \Gamma_{\theta} =& \left\{A\in\text{SL}(2,\mathbb{Z})\vert A\equiv \mathbb{1}_{2}\ \text{or}\  \mathbb{1}_{2}\ (\text{mod}\ 2)\right\},
    \end{split}
\end{align}
where $\text{SL}(2,\mathbb{Z})\supset \Gamma_{\theta}\supset \Gamma(2)$, and $\Gamma_{\theta}$ is called the theta group. The discrete subgroup $\Gamma(2)$ for example, is generated by $T^{2} = \left(\begin{smallmatrix}1 & 2\\ 0 & 1\end{smallmatrix}\right)$ and $ST^{2}S = \left(\begin{smallmatrix}-1 & \ 0\\ \ 2 & -1\end{smallmatrix}\right)$ which is denoted as $\Gamma(2) = \langle T^{2},ST^{2}S\rangle.$
There also exist special subgroups of the discrete group $\Gamma$ that we are interested in working with. These are called the congruence subgroups of level $N$ or the level $N$ principal congruence subgroups and are denoted by $\Gamma(N)$ with $N\in\mathbb{N}$. These are defined to be the identity mod $N$, i.e.
\begin{align}
    \begin{split} 
    \Gamma(N) =& \{\gamma\in\Gamma(1)\vert\ \gamma = \mathbb{1}_{2}\ (\text{mod}\ N)\}\\
    =& \left.\left\{\begin{pmatrix}
    a & b\\ c & d
    \end{pmatrix}\in\text{SL}(2,\mathbb{Z})\right\vert a\equiv d\equiv 1\  (\text{mod}\ N),\ b\equiv c\equiv 0\  (\text{mod}\ N)\right\},
   \end{split}
\end{align}
where $\Gamma(1) = \text{PSL}(2,\mathbb{Z})$ as noted earlier. A congruent subgroup of level $N$ is also a congruent subgroup of any multiple of $N$, i.e. $N' = \ell N$ for all $\ell\in\mathbb{N}$. The index of principal congruence subgroup $\Gamma(N)$ in $\text{SL}(2,\mathbb{Z})$ and in $\text{PSL}(2,\mathbb{Z})$ is given by
\begin{equation}\label{index}
      \begin{split}
          \mu =& \left[\text{SL}(2,\mathbb{Z}):\Gamma(N)\right]= N^{3}\prod\limits_{p\vert N}(1-p^{-2}),\\
          \overline{\mu} =& \left[\text{PSL}(2,\mathbb{Z}):\overline{\Gamma}(N)\right] = \begin{cases}
          \frac{1}{2}N^{3}\prod\limits_{p\vert N}(1-p^{-2}),\ N\geq 3,\\
          6,\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ N=2.
          \end{cases}
      \end{split}
\end{equation}
where $p\vert N$ denotes the prime divisors of $N$. Every congruence subgroup $\Gamma$ has a finite index in $\text{SL}(2,\mathbb{Z})$. There are several other special subgroups of $\Gamma$ of which the two most relevant for our discussion are $\Gamma_{0}(N)$ and $\Gamma_{1}(N)$, where the former is defined to be the subgroup of $\Gamma$ with matrices which have lower left entry $0$ mod $N$ and the latter is defined to the subgroup of $\Gamma$ with matrices that are identity except possibly in the upper right corner mod $N$. Explicitly, we have
\begin{align}\label{Hecke_subgroup}
    \begin{split}
    \Gamma_{0}(N) =& \left\{\left.\begin{pmatrix}
    a & b\\ c & d
    \end{pmatrix}\in\text{SL}(2,\mathbb{Z})\right\vert c\equiv 0\ (\text{mod}\ N)\right\} = \left\{\begin{pmatrix}
    * & *\\ 0 & *
    \end{pmatrix}\ \text{mod}\ N\right\},\\
    \Gamma_{1}(N) =& \left\{\begin{pmatrix}
    1 & *\\ 0 & 1
    \end{pmatrix}\text{mod}\ N\right\}.
    \end{split}
\end{align}
Here “$*$” stands for “unspecified”. These definitions satisfy
\begin{align}
    \Gamma(N)\subset\Gamma_{1}(N)\subset\Gamma_{0}(N)\subset\text{SL}(2,\mathbb{Z}).
\end{align}
We shall refer to $\Gamma_{0}(N)$ as Hecke subgroups from here on. When $N=1$, we have
\begin{equation}
    \text{SL}(2,\mathbb{Z}) = \Gamma_{0}(1) = \Gamma_{1}(1) = \Gamma(1).
\end{equation}
The index of the Hecke subgroup $\Gamma_{0}(N)$ in $\text{SL}(2,\mathbb{Z})$ and in $\text{PSL}(2,\mathbb{Z})$, and the index of the congruence subgroup $\Gamma_{1}(N)$ in $\text{SL}(2,\mathbb{Z})$ and in $\text{PSL}(2,\mathbb{Z})$ read \cite{Cohen_modular_forms}
\begin{align}\label{index_subgroups}
      \begin{split}
          \mu_{0} =& \left[\text{SL}(2,\mathbb{Z}):\Gamma_{0}(N)\right]= N\prod\limits_{p\vert N}(1+p^{-1}),\\
          \overline{\mu}_{0} =& \left[\text{PSL}(2,\mathbb{Z}):\overline{\Gamma}_{0}(N)\right] =  \begin{cases}
          N\prod\limits_{p\vert N}(1+p^{-1}),\ N\geq 3,\\
          3,\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ N=2,
          \end{cases}\\
          \mu_{1} =& \left[\text{SL}(2,\mathbb{Z}):\Gamma_{1}(N)\right]= \frac{N^{2}}{2}\prod\limits_{p\vert N}(1-p^{-2}),\\
          \overline{\mu}_{1} =& \left[\text{PSL}(2,\mathbb{Z}):\overline{\Gamma}_{1}(N)\right]= \begin{cases}
          \frac{N^{2}}{2}\prod\limits_{p\vert N}(1-p^{-2}),\ N\geq 3,\\
          3,\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ N=2.
          \end{cases}
      \end{split}
\end{align}
Additionally, we also have the following relations
\begin{align}\label{index_relations}
    \begin{split}
    &\left[\Gamma_{1}(N):\Gamma(N)\right] = N,\\
    &\left[\overline{\Gamma}_{1}(N):\overline{\Gamma}(N)\right] = N,\ N>2\\
    &\left[\Gamma_{1}(N):\Gamma(N^{2})\right] = N,\\
    &\left[\overline{\Gamma}_{1}(N):\overline{\Gamma}(N^{2})\right] = N,\ N>2\\
    &\left[\Gamma_{0}(N):\Gamma_{1}(N)\right] = \phi(N),\\
    &\left[\overline{\Gamma}_{0}(N):\overline{\Gamma}_{1}(N)\right] = \frac{1}{2}\phi(N),\ N>2\\
    &\left[\text{PSL}(2,\mathbb{Z}):\overline{\Gamma}_{1}(N^{2})\right] = \left[\text{PSL}(2,\mathbb{Z}):\overline{\Gamma}_{0}(N^{2})\right] = \left[\text{PSL}(2,\mathbb{Z}):\overline{\Gamma}(N)\right] = \frac{N^{3}}{2}\prod\limits_{p\vert N}\left(1 - p^{-2}\right),\ N\geq 3
    \end{split}
\end{align}
where Here, $\phi$ is the Euler's totient or Euler's phi function defined as follows
\begin{align}\label{Euler_totient}
    \phi(N) = N\prod\limits_{p\vert N}\left(1 - \frac{1}{p}\right),\ p\in\mathbb{P},
\end{align}
where the product is over the distinct prime numbers dividing $N$. The index is multiplicative, i.e. suppose $A,B,C$ are groups such that $A\subset B\subset C$ and the indices $[A:B]$ and $[B:C]$ are finite, then we have
\begin{align}
    [A:C] = [A:B][B:C].
\end{align}
For example, at level $N=7$, we have $\left[\Gamma_{1}(7):\Gamma(7)\right] = 7$, $\left[\Gamma_{0}(7):\Gamma_{1}(7)\right] = \phi(7) = 6$, $\left[\text{SL}(2,\mathbb{Z}:\Gamma_{0}(7)\right] = 7\prod\limits_{p\vert 7}\left(1+p^{-1}\right) = 8$. Using the multiplicative nature of the index, we find
\begin{align}
    \begin{split}
        \left[\text{SL}(2,\mathbb{Z}):\Gamma_{0}(7)\right]\left[\Gamma_{0}(7):\Gamma_{1}(7)\right]\left[\Gamma_{1}(7):\Gamma(7)\right] = 336 = \left[\text{SL}(2,\mathbb{Z}):\Gamma(7)\right],
    \end{split}
\end{align}
which matches with the result obtain using definition \ref{index}. For the Hall divisor $\ell\vert N$, i.e. in addition to $\ell$ being a divisor, $\ell$ and $\tfrac{N}{\ell}$ are coprime, the Atkin-Lehner involution at $\ell$ is defined to any matrix that has the following form
\begin{align}
    A_{\ell} = \frac{1}{\sqrt{\ell}}\begin{pmatrix}
    \ell\cdot a & b\\ N c& \ell\cdot d
  \end{pmatrix}
\end{align}
for $a,b,c,d\in\mathbb{Z}$ such that $\text{det}\ A_{\ell} =1$. These operators define involutions on the space of weakly holomorphic modular forms of weight $k$ denoted by $\mathcal{M}_{k}^{!}(\Gamma_{0}(N))$. Products of these involutions correspond to cusps of the Hecke group $\Gamma_{0}(N)$, and slashing by these matrices yield expansions at those cusps. The Atkin-Lehner involutions can be chosen such that they square to the identity matrix $\mathbb{1}_{2}$ and hence, they act as involutions when considered as modular transformations on the upper half-plane $\mathbb{H}^{2}$. For the special case of $k = N$, this is called the Fricke involution,
\begin{align}\label{Fricke_involution}
   \begin{split}
       W_{N} = \frac{1}{\sqrt{N}}\begin{pmatrix}
  0 & -1\\ N & 0
   \end{pmatrix},\\
   W_{N}:\tau\mapsto -\frac{1}{N\tau}.
   \end{split}
\end{align}
Let $[\tau]$ denote the equivalence class of $\tau\in\mathbb{H}^{2*}$ under the action of the group $\Gamma$ on $\mathbb{H}^{2}$. The Fricke involution exchanges two cusp classes $[i\infty]$ and $[0]$ while fixing the fixed point. For a positive integer $N$, the Fricke group denoted by $\Gamma^{+}_{0}(N)$ is generated by the Hecke group $\Gamma_{0}(N)$ and the Fricke involution $W_{N}$, i.e. $\Gamma_{0}^{+}(N) = \langle\Gamma_{0}(N),W_{N}\rangle$ or
\begin{equation}\label{Fricke}
    \Gamma_{0}^{+}(N) \equiv \Gamma_{0}(N)\cup \Gamma_{0}(N)W_{N}.
\end{equation}
The group $\Gamma_{0}^{*}(N)$ on the other hand, is one that is generated by the Hecke group and the Atkin-Lehner involution, i.e.
$\Gamma_{0}^{*}(N) = \langle\Gamma_{0}(N),A_{N}\rangle$. When $N \leq 5$ and when $N = p\in\mathbb{P}$, $\Gamma_{0}^{*}(N) = \Gamma_{0}^{+}(N)$. Let $M\in\mathbb{N}$ and let $h$ be the largest divisor of $24$ such that $M = Nh^{2}$. The normalizer of $\Gamma_{0}(m)$ is given by
\\
\begin{align}
    \mathcal{N}\left(\Gamma_{0}(m)\right) = \Gamma_{0}^{+}(Nh\vert h) = \begin{pmatrix} h & 0\\ 0 & 1\end{pmatrix}^{-1}\Gamma_{0}^{+}(N)\begin{pmatrix} h & 0\\ 0 & 1\end{pmatrix},
\end{align}
\\
where we notice that we recover the Fricke group when $h=1$. 
\begin{tcolorbox}[colback=blue!5!white,colframe=gray!75!black,title=]
  \begin{theorem}[\cite{Apostol}]\label{thm:Apostol_eta}
  For $\gamma = \left(\begin{smallmatrix}a & b\\ c & d\end{smallmatrix}\right)\in\text{SL}(2,\mathbb{Z})$ with $c>0$ and $\tau\in\mathbb{H}^{2}$,
    \begin{align}
      \begin{split}
          \eta(\gamma(\tau)) =& \eta\left(\frac{a\tau + b}{c\tau + d}\right) = \epsilon(a,b,c,d)\left(-i(c\tau + d)\right)^{\frac{1}{2}}\eta(\tau),\\
          \epsilon(a,b,c,d) =& \text{exp}\left[\pi i\left(\frac{a+d}{12c} + s(-d,c)\right)\right],\\
          s(a,b)=& \sum\limits_{\ell=1}^{b-1}\frac{\ell}{b}\left(\frac{a\ell}{b} - \left\lfloor\left.\frac{a\ell}{b}\right\rfloor\right. - \frac{1}{2}\right).
      \end{split}
  \end{align}
  \end{theorem}
\end{tcolorbox}
\noindent
It follows from this theorem that if $k\vert N$ and $\gamma = \left(\begin{smallmatrix}a & b\\ Nc & d\end{smallmatrix}\right)\in\Gamma_{0}(N)$ with $c>0$, then 
\begin{align}
    \begin{split}
        \eta(k\gamma(\tau)) =& \eta\left(\frac{ka\tau + kb}{Nc\tau + d}\right) = \eta\left(\begin{pmatrix}
        a & kb\\ Nc & d
        \end{pmatrix}(k\tau)\right)\\
        =& \epsilon\left(a,kb,\tfrac{cN}{k},d\right)\left(-i(Nc\tau + d)\right)^{\frac{1}{2}}\eta(k\tau).
    \end{split}
\end{align}
Under the $S$-transform, the Dedekind eta-function behaves as follows
\begin{align}\label{Dedekind_S_transform}
    \begin{split}
        \eta(S(\tau)) =& (-i\tau)^{\tfrac{1}{2}}\eta(\tau),\\
        \eta(N\cdot S(\tau)) =& \left(-\frac{i\tau}{N}\right)^{\tfrac{1}{2}}\eta\left(\frac{\tau}{N}\right).
    \end{split}
\end{align}


\subsection*{Signature and genus of congruence subgroups}
We consider a somewhat larger set of congruence subgroups described by
\begin{equation}
    H(p,q,r;\chi,\tau) = \left\{\left.\begin{pmatrix}
    1 + ap & bq\\ cr & 1 + dp
    \end{pmatrix} \in \Gamma\right\vert a,b,c,d\in\mathbb{Z},\ c\equiv \tau a\ (\text{mod}\ \chi)\right\},
\end{equation}
where $p$ divides $qr$ and $\chi$ divides $\text{gcd}\left(p,\tfrac{qr}{p}\right)$. These groups include $\Gamma(N) = H(N,N,N;1,1)$, the Hecke subgroup $\Gamma_{0}(N) = H(1,1,N;1,1)$, and $\Gamma_{1}(N) = H(N,1,N;1,1)$. A subgroup of $\Gamma$ is called a regular subgroup if it contains $I  = \mathbb{1}_{2}$, the identity element of $\Gamma$. If a subgroup is not regular, it is called irregular. In general, the subgroup $H(p,q,r;\chi,\tau)$ is irregular and the associated regular subgroup is denoted by $\pm H(p,q,r;\chi,\tau)$. Let $H(p,N;\chi) = H(p,N,1;\chi,1)$, for $p,N,\chi\in\mathbb{Z}$ such that $p\vert N$ and $\chi\vert \text{gcd}\left(p,\tfrac{N}{p}\right)$. 
\begin{tcolorbox}[colback=magenta!5!white,colframe=gray!75!black,title=]
  \begin{lemma}[\cite{Cummins}]
    For $p,q,r,\chi,\tau\in\mathbb{Z}_{+}$, such that $p\vert qr$and $\chi\vert\text{gcd}\left(p,\tfrac{qr}{p}\right)$. Let $g = \text{gcd}(\chi,\tau)$. Then the groups $H(p,q,r;\chi,\tau)$ and $H(p,gqr;\chi/g)$ have the same signatures. 
  \end{lemma}
\end{tcolorbox}
\noindent
Let $\Gamma'$ be a subgroup of finite index $\mu = \mu(\Gamma')$ of the modular group $\Gamma$ or in other words, $\Gamma'$ can be described as a finitely generated Fuchsian group of the first kind contained in $\Gamma$. Then, the index $\mu = [\text{SL}(2,\mathbb{Z}): \Gamma(N)]$ defined in \ref{index} is given by the following formula
\begin{equation}\label{index_euler_char}
    \mu = \frac{\text{Area}(\Gamma'\backslash\mathbb{H}^{2})}{\text{Area}(\Gamma\backslash\mathbb{H}^{2})} = 6\left(2g-2 + \sum\limits_{j=1}^{v}\left(1 - \frac{1}{m_{j}}\right)\right) = 6\chi(\Gamma'),
\end{equation}
where $\chi(\Gamma')$ is the (negative) Euler characteristic of $\Gamma'$. The group $\Gamma$ contains elliptic elements of orders $2$ and $3$ only. Hence, let us define the following
\begin{itemize}
    \item $\nu_{0} = \nu_{0}(\Gamma')$ be the degree of covering of Riemann surfaces $X(\Gamma')\to X(\Gamma)$ given by the index of the subgroup $\Gamma'$ in $\Gamma$, i.e.
    \begin{equation}
        \nu_{0}(\Gamma') = \mu(\Gamma'),
    \end{equation}
    \item $\nu_{2} = \nu_{2}(\Gamma')$ be the number of $\Gamma'$-inequivalent elliptic fixed points (in $\mathbb{H}^{2}$) of order $2$, 
    \item $\nu_{3} = \nu_{3}(\Gamma')$ be the number of $\Gamma'$-inequivalent elliptic fixed points (in $\mathbb{H}^{2}$) of order $3$,
    \item $\nu_{\infty} = \nu_{\infty}(\Gamma')$ be the number of $\Gamma'$-inequivalent parabolic fixed points (in $\mathbb{Q}\cup \{\infty\}$) given by
    \begin{equation}
      \nu_{\infty}(\Gamma') = \nu_{\infty}^{\text{reg}}(\Gamma') + \nu_{\infty}^{\text{irr}},  
    \end{equation}
    where $\nu_{\infty}^{\text{reg}}(\Gamma')$ and $\nu_{\infty}^{\text{irr}}(\Gamma')$ are the number of regular and irregular cusps of $\Gamma'$ respectively. 
    \item If the discriminant $D$ of the imaginary quadratic field $K = \mathbb{Q}\left(\sqrt{-D}\right)$ is $5$, $8$, and $12$ then $\nu_{5}$, $\nu_{4}$, and $\nu_{6}$ respectively occur.
    \item If the discriminant $D$ of the imaginary quadratic field $K = \mathbb{Q}\left(\sqrt{-D}\right)$ is different from $5$, $8$, and $12$ then only $\nu_{2}$ and $\nu_{3}$ exist.
\end{itemize}
\noindent
\begin{tcolorbox}[colback=blue!5!white,colframe=gray!75!black,title=]
\begin{theorem}[\cite{Shimura}]\label{thm:genus}
  The genus of the curve $X(\Gamma') = \Gamma'\backslash\mathbb{H}^{2*}$ is
  \begin{equation}
      g(X(\Gamma')) = 1 + \frac{\nu_{0}(\Gamma')}{12} - \frac{\nu_{2}(\Gamma')}{4} - \frac{\nu_{3}(\Gamma')}{3} - \frac{\nu_{\infty}(\Gamma')}{2}. 
  \end{equation}
\end{theorem}
\end{tcolorbox}
\noindent 
\begin{tcolorbox}[colback=blue!5!white,colframe=gray!75!black,title=]
\begin{theorem}[\cite{Kok}]\label{thm:genus_Fricke_index}
  Let $\Gamma'$ be an intermediate group of $\Gamma_{0}(M)\leq \mathcal{N}\left(\Gamma_{0}(M)\right) = \Gamma_{0}(Nh\vert h)$, where $M\in\mathbb{N}$ and $M = Nh^{2}$ with $h$ as the largest divisor of $24$. The genus of the curve $X(\Gamma') = \Gamma'\backslash\mathbb{H}^{2}$ reads 
  \begin{equation}\label{genus_Fricke_eqn}
      g(X(\Gamma')) = 1 + \chi(\Gamma_{0}^{+}(N))\frac{\left[\Gamma_{0}^{+}(Nh\vert h):\Gamma'\right]}{2} -
       \frac{5\nu_{6}(\Gamma')}{12} - \frac{3\nu_{4}(\Gamma')}{8} - \frac{2\nu_{3}(\Gamma')}{6} - \frac{\nu_{2}(\Gamma')}{4} - \frac{\nu_{\infty}(\Gamma')}{2},
  \end{equation}
  where $\chi_{0}(\Gamma_{0}^{+}(M)) = \tfrac{M}{6}\prod\limits_{p\vert M}\tfrac{p+1}{2p}$ is the Euler characteristic.
\end{theorem}
\end{tcolorbox}
\noindent 
Let us consider $H$ to be one of the groups of the set $H(p,q,r;\chi,\tau)$ or $\pm H(p,q,r;\chi,\tau)$. The signature of $H$ is given by $(\mu,\nu_{2},\nu_{3},\nu_{\infty}^{\text{reg}},\nu_{\infty}^{\text{irr}})$ and the signature of $\pm H$ is given by $(\mu, \nu_{2},\nu_{3},\nu_{\infty}^{\text{reg}} + \nu_{\infty}^{\text{irr}}, 0)$. 
\begin{tcolorbox}[colback=blue!5!white,colframe=gray!75!black,title=]
  \begin{theorem}[\cite{Cummins}]\label{thm:reg_irr_cusps}
    For $p,q,r,\chi,\tau\in\mathbb{Z}_{+}$ such that $q\vert N$ and $\chi\vert \text{gcd}\left(p,\tfrac{N}{p}\right)$. Let $c = c(p,N;\chi)$ be the number of orbits of group $H(p,N;\chi)$ acting on a set related to the cups of $\Gamma(N)$. then, the number of regular and irregular cusps of $H(p,N;\chi)$ is given by
    \begin{align}
        \left(\nu_{\infty}^{\text{reg}},\nu_{\infty}^{\text{irr}}\right) = \begin{cases}
        (c,0),\ \text{if}\ p=2,\ \text{and}\ \chi = 1,\\
        \ \ \ \ \ \ \ \ \text{or}\ p=1,\\
        \left(\frac{2c}{5},\frac{c}{5}\right),\ \text{if}\ p=2,\ \chi = 2,\ 2\vert\vert (N/p),\\
        \left(\frac{c}{4},\frac{c}{2}\right),\ \text{if}\ p=2,\ \chi = 2,\ 2^{k}\vert\vert (N/p),\ k\ \text{odd},\ k>1\\
        \left(\frac{c}{3},\frac{c}{3}\right),\ \text{if}\ p=2,\ \chi = 2,\ 2^{k}\vert\vert (N/p),\ k\ \text{even}\\
        \left(\frac{2c}{5},\frac{c}{5}\right),\ \text{if}\ p=4,\ \chi = 2,\ 2\nmid (N/p),\ (\text{so}\ \chi=1)\\
        \left(\frac{c}{2},0\right),\ \text{otherwise}
        \end{cases}
    \end{align}
  \end{theorem}
\end{tcolorbox}
\noindent
Here, we have used the notation $a\vert\vert b$ for $a,b,\in\mathbb{Z}$ that is to be read as $a$ exactly divides $b$ and $\text{gcd}(a,b)=1$.
\\
\begin{tcolorbox}[colback=blue!5!white,colframe=gray!75!black,title=]
  \begin{theorem}\label{thm:eliptic_points}
    The number of elliptic points of order $2$ for $\Gamma_{0}(N)$ is given by 
    \begin{align}
        \begin{split}
            \nu_{2}(\Gamma_{0}(N)) = \begin{cases} \prod\limits_{p\vert N}\left(1 + \left(\frac{-1}{p}\right)\right),\ &\text{if}\ 4\nmid N,\\
            0,\ &\text{if}\ 4\vert N,
        \end{cases}
        \end{split}
    \end{align}
    where $\left(\tfrac{-1}{p}\right) = \pm 1$ if $p = \pm 1(\text{mod}\ 4)$ and is $0$ if $p = 2$, and the number of elliptic points of order $3$ for $\Gamma_{0}(N)$ is given by 
    \begin{align}
         \begin{split}
            \nu_{3}(\Gamma_{0}(N)) = \begin{cases} \prod\limits_{p\vert N}\left(1 + \left(\frac{-3}{p}\right)\right),\ &\text{if}\ 9\nmid N,\\
            0,\ &\text{if}\ 9\vert N,
        \end{cases}
        \end{split}
    \end{align}
     where $\left(\tfrac{-3}{p}\right) = \pm 1$ if $p = \pm 1(\text{mod}\ 3)$ and is $0$ if $p = 3$.
  \end{theorem}
\end{tcolorbox}
\noindent
\begin{tcolorbox}[colback=orange!5!white,colframe=gray!75!black,title=]
  \begin{prop}\label{prop:identity_element}
  The cases when $H(p,q,r;\chi,\tau)$ contains the identity element $I = \mathbb{1}_{2}$ are
  \begin{enumerate}
      \item $p=2,\ \chi = 2,\ \tau$ even.
      \item $p = 2,\ \chi=1$.
      \item $p=1,\ \chi = 1$.
  \end{enumerate}
  \end{prop}
\end{tcolorbox}
\noindent
For the case of Hecke subgroups $\Gamma_{0}(k)$ defined in \ref{Hecke_subgroup} with $k$ an odd prime, we have
\begin{align}
    \mu =& k+1,\ \ \nu_{\infty} = 2,\\
    \nu_{2} =& \begin{cases}
     2,\ \text{if}\ k\equiv 1(\text{mod}\ 4),\\ 0,\ \text{if}\ k\equiv 3(\text{mod}\ 4),
    \end{cases}\\
    \nu_{3} =& \begin{cases}
    1,\ \text{if}\ k = 3\\
    2,\ \text{if}\ k\equiv 1(\text{mod}\ 3),\\
    0,\ \text{if}\ k\equiv 2(\text{mod}\ 3).\\
    \end{cases}
\end{align}
The genus for $k=p$ prime reads
\begin{equation}
    g(\Gamma_{0}(p)) = \begin{cases}
    0,\ \text{if}\ p=2\ \text{and}\ 3,\\
    \frac{p-13}{12},\ \text{if}\ p\equiv 1(\text{mod}\ 12),\\
    \frac{p-n}{12},\ \text{if}\ p\equiv n(\text{mod}\ 12)\ \text{for}\ n=5\ \text{and}\ 7,\\
    \frac{p+1}{12},\ \text{if}\ p\equiv 11(\text{mod}\ 12).
    \end{cases}
\end{equation}
The (negative) Euler characteristic for $k$ prime is given by 
\begin{equation}
    \chi = \frac{k+1}{6}. 
\end{equation}
For the case of the Fricke group $\Gamma^{+}_{0}(p) = \Gamma^{*}_{0}(p)$ where $p$ is $1$ or a prime for which the genus of $\Gamma_{0}^{+}(p)$ is zero, i.e. $p\in\{1,2,3,5,7,11,13,17,19,23,29,31,41,47,59,71\}$.
\\
\begin{tcolorbox}[colback=magenta!5!white,colframe=gray!75!black,title=]
  \begin{lemma}[\cite{Choi}]\label{lemma:Fixed_points}
   The number of fixed points $\#$ of the Frick involution $W_{p}$ on $X_{0}(p)$ is given by 
   \begin{align}
       \begin{split}
           \# = \begin{cases}
           \tfrac{p-1}{6},\ &p\equiv 1(\text{mod}\ 12),\\
           \tfrac{p+7}{6},\ &p\equiv 5(\text{mod}\ 12),\\
           \tfrac{p+5}{6},\ &p\equiv 7(\text{mod}\ 12),\\
           \tfrac{p+13}{6},\ &p\equiv 11(\text{mod}\ 12),\\
           \end{cases}
       \end{split}
   \end{align}
   \end{lemma}
\end{tcolorbox}
\noindent
The genus of $\Gamma_{0}^{+}(p)$ reads
\begin{equation}\label{genus_Fricke}
    g(\Gamma^{+}_{0}(p)) = \frac{1}{4}\left(g(\Gamma_{0}(p)) + 2 - \#)\right).
\end{equation}


\subsection*{The dimension of spaces of forms of congruent subgroups}
We state useful theorems that provide us with a working formula to find the dimensions spaces of forms. Let $\mathcal{M}_{k}(\Gamma')$ and $\mathcal{S}_{k}(\Gamma')$ be the space of modular forms and the space of cusp forms of the congruent subgroup $\Gamma'$ respectively.
\section*{Case I: $\Gamma'\subseteq\Gamma$}
\begin{tcolorbox}[colback=blue!5!white,colframe=gray!75!black,title=]
\begin{theorem}[\cite{Shimura}]\label{thm:space_dim_G}
   If $k\geq 2$ is even, then the dimension of the space of cusp forms of $\Gamma'$ and the space of modular forms is
  \begin{align}
      \begin{split}
          \text{dim}\ \mathcal{S}_{k}(\Gamma') =& \delta_{2,k} + \frac{k-1}{12}\nu_{0}(\Gamma') + \left(\left\lfloor\left.\frac{k}{4}\right\rfloor\right. - \frac{k-1}{4}\right)\nu_{2}(\Gamma')\\
          +& \left(\left\lfloor\left.\frac{k}{3}\right\rfloor\right. - \frac{k-1}{3}\right)\nu_{3}(\Gamma') - \frac{\nu_{\infty}(\Gamma')}{2},\\
      \text{dim}\ \mathcal{M}_{k}(\Gamma') =& \text{dim}\ \mathcal{S}_{k}(\Gamma') + \nu_{\infty}(\Gamma')  - \delta_{2,k}.
      \end{split}
  \end{align}
  If $k\geq 3$ is odd and $-I\notin \Gamma'$, then 
   \begin{align}
      \begin{split}
          \text{dim}\ \mathcal{S}_{k}(\Gamma') =&  \frac{k-1}{12}\nu_{0}(\Gamma') + \left(\left\lfloor\left.\frac{k}{3}\right\rfloor\right. - \frac{k-1}{3}\right)\nu_{3}(\Gamma')  - \frac{\nu_{\infty}^{\text{reg}}(\Gamma')}{2},\\
      \text{dim}\ \mathcal{M}_{k}(\Gamma') =& \text{dim}\ \mathcal{S}_{k}(\Gamma') + \nu_{\infty}^{\text{reg}}(\Gamma'),
      \end{split}
  \end{align}
  and the spaces $\mathcal{M}_{k}(\Gamma')$ are trivial for $k$ odd when $-I\in \Gamma'$. 
\end{theorem}
\end{tcolorbox}
\noindent 

\section*{Case II: $\Gamma' = \Gamma_{H}(N)\subseteq\Gamma$}
\begin{tcolorbox}[colback=blue!5!white,colframe=gray!75!black,title=]
    \begin{theorem}[\cite{Cohen-I}]\label{thm:space_dim_G_0}
    Consider the congruence subgroups $\Gamma'\subset\Gamma$ defined by \begin{equation}
    \Gamma_{H}(N) = \left\{\left.\begin{pmatrix}
    a & b\\ c & d
    \end{pmatrix}\in\text{SL}(2,\mathbb{Z})\right\vert c\equiv 0(\text{mod}\ N),\ a,\ d\in H\right\}
    \end{equation}
    for $H$ a subgroup of the multiplicative group $(\mathbb{Z}/N\mathbb{Z})^{*}$. this includes two cases $\Gamma_{1}(N)$ and $\Gamma_{0}(N)$ corresponding to groups $H = \{1\}$ and $H = (\mathbb{Z}/N\mathbb{Z})^{*}$ respectively. Then, the dimension of the space of cusp forms and modular forms read 
    \begin{align}
        \begin{split}
            \text{dim}\ \mathcal{S}_{k}(\Gamma_{H}(N)) =& 2\left\lfloor\left. \frac{k}{3}\right\rfloor\right.-1 \ \text{if}\ k\geq 3,\\ \text{dim}\ \mathcal{M}_{k}(\Gamma_{H}(N)) =& 2\left\lfloor\left. \frac{k}{3}\right\rfloor\right.+1 \ \text{if}\ k\geq 1.
        \end{split}
    \end{align}
  \end{theorem}
\end{tcolorbox}
\noindent 

\section*{Case III: $\Gamma' = \Gamma^{+}_{0}(N)$}
\begin{tcolorbox}[colback=blue!5!white,colframe=gray!75!black,title=]
\begin{theorem}[\cite{Choi}]\label{thm:space_dim_G*0}
   For $k> 2$ with $k$ being an even integer, the dimension of the space of cusp forms of $\Gamma'$ is
  \begin{align}
      \begin{split}
          \text{dim}\ \mathcal{S}_{k}(\Gamma^{+}_{0}(2)) =&  \begin{cases}
          \left\lfloor\left.\frac{k}{8}\right\rfloor\right. - 1,\ k\equiv 2 (\text{mod}\ 8)\\
          \left\lfloor\left.\frac{k}{8}\right\rfloor\right.,\ \ \ \ \ \ k\equiv 2(\text{mod}\ 8),\\
          \end{cases}\\
          \text{dim}\ \mathcal{S}_{k}(\Gamma^{+}_{0}(3)) =& \begin{cases}
          \left\lfloor\left.\frac{k}{6}\right\rfloor\right.-1,\ k\equiv 2,6(\text{mod}\ 12),\\
          \left\lfloor\left.\frac{k}{6}\right\rfloor\right.,\ \ \ \ \ \  k\not\equiv 2,6(\text{mod}\ 12),\\
          \end{cases}\\
          \text{dim}\ \mathcal{S}_{k}(\Gamma^{+}_{0}(p)) =& \begin{cases}
          \left(\tfrac{p+5}{6}\right)\left\lfloor\left.\frac{k}{4}\right\rfloor\right. + \left\lfloor\left.\frac{k}{3}\right\rfloor\right. - \frac{k}{2},\ p\equiv 1,7(\text{mod}\ 12),\\
          \left(\tfrac{p + 13}{6}\right)\left\lfloor\left.\frac{k}{4}\right\rfloor\right. - \frac{k}{2},\ \ \ \ p \equiv 5,11(\text{mod}\ 12),
          \end{cases}
      \end{split}
  \end{align}
  where the third expression is for $p>3$. The dimension of the space of modular forms is 
  \begin{align}
    \text{dim}\ \mathcal{M}_{k}(\Gamma^{+}_{0}(p)) = 1 + \text{dim}\ \mathcal{S}_{k}(\Gamma^{+}_{0}(p)),    
  \end{align}
  for $p\in\{1,2,3,5,7,11,13,17,19,23,29,31,41,47,59,71\}$.
\end{theorem}
\end{tcolorbox}
\noindent
We follow \cite{Junichi} for finding the basis decomposition of spaces of modular forms and valence formulae of various Fricke and Hecke groups.
\noindent 



==> Other_groups.tex <==
\section{Other groups}\label{sec:other_groups}
Investigation for single character solutions in the Hecke groups of levels $N\leq 12$ did not reveal any admissible solutions. In the previous section, we found quasi-characters in $\Gamma_{0}(7)$. We see this repeat in the solutions of the $\Gamma_{0}(2)$ which we then use to construct the admissible solutions of $\Gamma_{0}^{+}(2)$. After this, we consider $\Gamma_{0}(3)$ as an example and present the single character analysis to elucidate some of the issues that make the solution inadmissible in the other Hecke group levels. What about Fricke groups of other levels? It turns out that there are no admissible single character solutions for $\Gamma_{0}^{+}(N)$ with $N\leq 12$ except at $N = 2,3,5,7$ which are all genus zero Moonshine groups and are the first four prime divisors of $\mathbb{M}$. 
%It is surprising that this feature of admissible solutions is not shared with the group $\Gamma_{0}^{+}(11)$ which is also a genus zero Moonshine group.

\input{Gamma_0_2}
\input{Gamma_0_3}
\input{Gamma_1_N}
%\input{Other_subgroups}
%\input{Gamma_0_4}
%\input{Gamma_0_4+}


==> Three_character_Gamma_0_2+.tex <==
\section{Three-character theories (note: section yet to be completed)}
Let us now consider three character theories with $\ell = 0$. The modular invariant differential equation reads
\begin{align}
    \left[\omega_{0}(\tau)\mathcal{D}^{3} + \omega_{2}(\tau)\mathcal{D}^{2} + \omega_{4}(\tau)\mathcal{D} + \omega_{6}(\tau)\right]f(\tau) = 0.
\end{align}
Since there are no modular forms of weight $2$ in $\Gamma_{0}^{+}(2)$, with choices $\omega_{4}(\tau) =\mu_{1} E_{4}^{(2^{+})}(\tau)$ and $\omega_{6}(\tau) = \mu_{2} E_{6}^{(2^{+})}(\tau)$ and in terms of derivatives $\Tilde{\partial}$, the MLDE reads
\begin{align}
        \left[\Tilde{\partial}^{3} - \frac{1}{6}\left(\Tilde{\partial}E_{2}(\tau)\right)\Tilde{\partial}  - \frac{1}{2}E_{2}\Tilde{\partial}^{2} + \frac{1}{18}E^{2}_{2}\Tilde{\partial} + \mu_{1}E_{4}^{(2^{+})}(\tau)\Tilde{\partial} + \mu_{2}E_{6}^{(2^{+})}(\tau)\right]f(\tau) = 0.
\end{align}
We now make use of the Ramanujan identity for the Eisenstein series, $\Tilde{\partial}E_{2} = \tfrac{E_{2}^{2} - E_{4}}{12}$, to rewrite the MLDE as follows
\begin{align}
    \left[\Tilde{\partial}^{3} + \frac{1}{2}\left(\Tilde{\partial}E_{2}(\tau)\right)\Tilde{\partial}  - \frac{1}{2}E_{2}(\tau)\Tilde{\partial}^{2} + \frac{1}{18}E_{4}(\tau)\Tilde{\partial} + \mu_{1}E_{4}^{(2^{+})}(\tau)\Tilde{\partial} + \mu_{2}E_{6}^{(2^{+})}(\tau)\right]f(\tau) = 0.
\end{align}
We make the following mode expansion substitutions for $f(\tau)$, and the modular forms in the above MLDE
\begin{align}
    \begin{split}
        f(\tau) =& q^{\alpha}\sum\limits_{n= 0}^{\infty}f_{n}q^{n},\\ 
         E_{k}(\tau) =& \sum\limits_{n=0}^{\infty}E_{k,n}q^{n},\\
         E_{4}^{(2^{+})}(\tau) =& \sum\limits_{n=0}^{\infty}E_{4,n}^{(2^{+})}q^{n}\\
        =& 1 + 48 q + 624 q^2 + 1344 q^3 + 5232 q^4 + \ldots,\\
        E^{(2^{+})}_{6}(\tau) =& \sum\limits_{n=0}^{\infty}E^{(2^{+})}_{6,n}q^{n}\\
        =& 1 - 56 q - 2296 q^2 - 13664 q^3 - 73976 q^4 + \ldots,\\
        \Tilde{\partial}E_{2}(\tau) =& q\frac{d}{dq}E_{2}(\tau) = \sum\limits_{n = 0}^{\infty}\mathfrak{e}_{n}q^{n}\\
        =& 24 q - 144 q^2 - 288 q^3 - 672 q^4 - 720 q^5 + \ldots
    \end{split}
\end{align}
We now have the recursion relation
\begin{align}\label{m_1_equation}
    \begin{split}
    &\left((n + \alpha)^{3} - \frac{1}{2}(n + \alpha)^{2} + \left(\mu_{1} + \frac{1}{18}\right)(n + \alpha) + \mu_{2}\right)f_{n} =\\ &\sum\limits_{m=1}^{n}\left(\frac{(n + \alpha - m)^{2}}{2}E_{2,m}
    - \left(\frac{1}{2}\mathfrak{e}_{m} + \frac{1}{18}E_{4,m} + \mu_{1}E^{(2^{+})}_{4,m}\right) (n + \alpha - m) - \mu_{2}E^{(2^{+})}_{6,m}\right)f_{n-m}.
    \end{split}
\end{align}
For $n = 0$, we get the equation
\begin{align}\label{indicial_cubic}
    \alpha^{3} - \frac{1}{2}\alpha^{2} + \Tilde{\mu}_{1}\alpha + \mu_{2} = 0,
\end{align}
where we have defined $\Tilde{\mu}_{1}\equiv \mu_{1} + \tfrac{1}{18}$. For $n = 1$, we obtain the following ratio
\begin{align}\label{m_1_finding_equation}
    \left(3\alpha^{2} + 2\alpha + \frac{5}{9} + \mu_{1}\right)m_{1} + \left(56\alpha^{3} - 16\alpha^{2} + 104\alpha\mu_{1} - \frac{40}{9}\alpha\right) = 0,
\end{align}
where $ m_{1} \equiv \tfrac{f_{1}}{f_{0}}$. From these equations, we find
\begin{align}
    \begin{split}
        \mu_{1} =& \alpha_{0}\alpha_{1} + \alpha_{1}\alpha_{2} + \alpha_{0}\alpha_{2} - \frac{1}{18},\\
        \mu_{2} =& -\alpha_{0}\alpha_{1}\alpha_{2},
    \end{split}
\end{align}
where $\alpha_{i}$ with $i=0,1,2$ are the roots of the cubic equation. With $\mu_{2}$ obtained through the indicial cubic equation, we find the following explicit expression for $\mu_{1}$ from \ref{m_1_equation}
\begin{align}
    \mu_{1} = -\frac{504 \alpha_{0}^{3} + \alpha_{0}^{2}(27m_{1} - 144) + \alpha_{0}(40 + 18m_{1}) + 5m_{1}}{9(m_{1} + 104\alpha_{0})}.
\end{align}
We now consider the outcome of the recursion relation for $n =2$ and substitute the known expressions of $\mu_{1}$ and $\mu_{2}$ to obtain
\begin{align}
    \begin{split}
        0 &=225792\alpha_{0}^{4} + \alpha_{0}^{3}\left(-206784 - 27456m_{1} - 768m_{1}^{2} + 1536m_{2}\right)\\
        &+ \alpha_{0}^{2}\left(15840 - 11064m_{1} - 1104m_{1}^{2} + 3216m_{2}\right)\\
        &+ \alpha_{0}(-820m_{1} - 376m_{1}^{2} + 1880m_{2}+ 18m_{1}m_{2}) - (40m_{1}^{2} - 15m_{1}m_{2}).
    \end{split}
\end{align}
We observe that if we define the variable 
\begin{align}\label{N_def}
    N = -28224\alpha_{0},
\end{align}
then the polynomial equation simplifies to 
\begin{align}\label{poly_quartic}
    \begin{split}
        0 &= N^{4} + \left(25848 + 3432m_{1} + 96m_{1}^{2} - 192m_{2}\right)N^{3}\\ &+\left(55883520 - 39033792m_{1} - 3894912m_{1}^{2}+11346048m_{2}\right)N^{2}\\
        &+ \left(81650903040m_{1} + 37439926272m_{1}^{2} -187199631360m_{2}-1792336896m_{1}m_{2}\right)N\\ 
        &- \left(112415370117120m_{1}^{2} - 42155763793920m_{1}m_{2}\right).
    \end{split}
\end{align}
The integer-root theorem requires $N$ to be an integer. Hence, $N$ is further restricted- it not only has to be rational but also is to be an integer. Since $\alpha_{0} = -\tfrac{c}{24}$, we obtain the relation $c = \tfrac{N}{1176}$ from which we see that the central charge has to be a rational number whose denominator is always $1176$. Substituting $\mu_{1}$ and $\mu_{2}$ in \ref{indicial_cubic}, with the definition of $N$ in \ref{N_def} we get
\begin{align}
    \begin{split}
    0 &=\left(\alpha+\frac{N}{28224}\right)\left((1725954048 N - 468397375488m_{1})\alpha^{2} \right.\\
    &\left.+ (-862977024 N - 61152 N^2 + 234198687744m_{1} + 16595712 N m_{1})\alpha\right.\\
    &\left.+(1176 N^{2}m_{1} - 41489280 Nm_{1} + 234198687744 + N^{3} + 21168N^{2} + 22127616 N)\right).
    \end{split}
\end{align}
We see from this that $\alpha = \alpha_{0} = -\tfrac{N}{28224}$ is one of the solutions. Let us denote the other solutions by $\alpha_{1}$ and $\alpha_{2}$ so that $\alpha_{1} - \alpha_{0}$, and $\alpha_{2} - \alpha_{0}$ are the conformal weights $\Delta_{1}$ and $\Delta_{2}$. Hence, $\alpha_{1}$ and $\alpha_{2}$ should also be rational which implies that the discriminant, which is an integer, has to be the perfect square to be able to result in rational roots. This yields
\begin{align}\label{k_equation}
    \begin{split}
        k^{2} = &22308830199742464m_{1}^{2} - 89463898718208m_{1} N - 3161682284544 m_{1}^{2}N + 26752287744 N^{2}\\
        &+ 12148061184 m_{1}N^{2} + 
        112021056m_{1}^{2}N^{2} - 1834560N^{3} - 373968m_{1}N^{3} - 143N^{4},
    \end{split}
\end{align}
where $k$ is a positive integer. This equation where all the unknown variables $N$, $m_{1}$, and $k$ are positive is known as a Diophantine equation. The roots are found to be
\begin{align}
    \frac{-49787136m_{1} + 183456 N -3528 m_{1}N + 13N^{2} \pm k}{56448(13 N - 3528 m_{1})},
\end{align}
where the smaller solution corresponds to $\alpha_{1}$ and the larger one corresponds to $\alpha_{2}$. We now solve \ref{poly_quartic} for a fixed value of $N$ (chosen among the divisors of $28224$) and obtain the solution set $(N,m_{1},m_{2})$. Now, we choose those values of $m_{1}$ and $N$ that result in positive integer values for $k$ that satisfies \ref{k_equation}. By following this procedure, we would have found values for $N$, $m_{1}$, $m_{2}$, and $k$, all of which simultaneously solve equations \ref{poly_quartic} and \ref{k_equation}. The only solution we could find was at $N = 14112$ for which we obtain the values listed in table \ref{tab:N_value}
\\
\begin{table}[htb!]
    \centering
    \begin{tabular}{c|c|c|c}
    $N$ & $m_{1}$ & $m_{2}$ & $k$\\
    \hline & & & \\
    %7056 & 34 & 5 & \\
    14112 & 58 & 66 & 796594176\\
    \end{tabular}
    \caption{Simultaneous solution for $0< N\leq 28224$.}
    \label{tab:N_value}
\end{table}
\\
For the above values, we find roots
\begin{align}
    (\alpha_{0},\alpha_{1},\alpha_{2}) = \left(-\frac{1}{2},-\frac{1}{6},\frac{7}{6}\right).
\end{align}
From this we find central charge and conformal dimensions $(c,\Delta_{1},\Delta_{2}) = \left(12,\tfrac{1}{3},\frac{5}{3}\right)$, and free parameters $(\mu_{1},\mu_{2}) = \left(-\tfrac{25}{36},-\tfrac{7}{72}\right)$. Thus far, we have only investigated the vacuum character and found the $q$-series expansion 
\begin{align}
    \chi_{0}(\tau) = q^{-\tfrac{1}{2}}\left(1 + 58q + 66q^{2} + \ldots\right).
\end{align}
In order to establish that this is indeed a valid character, we should check for positivity in higher-order Fourier coefficients and repeat the same process for the characters $\chi_{\tfrac{1}{3}}(\tau)$ and $\chi_{\tfrac{5}{3}}(\tau)$ in order to rule this as an admissible solution. The following is a general expression we obtain for the ratio $m_{1}$ from \ref{m_1_finding_equation},
\begin{align}
    m_{1}^{(i)} \equiv \frac{f_{1}^{(i)}}{f_{0}^{(i)}} = \ldots
\end{align}
where $i = 0,1,2$. From this we find $m_{1}^{(1)} = \ldots$








==> Two_character_Gamma_0_7+.tex <==
\section{Two-character theories for \texorpdfstring{$\Gamma_{0}^{+}(7)$}{Γ0(7)+}}\label{appendix:D}
For the general form of the MLDE for $n=2$, the free parameters $\mu_{i}$ come as coefficients to the modular forms and the number of them can be determined as follows
\begin{align}\label{number_of_parameters_F}
    \begin{split}
        \#(\mu) =&\text{dim}\mathcal{M}_{2\ell}(\Gamma^{+}_{0}(7)) + \text{dim}\mathcal{M}_{2\ell + 2}(\Gamma^{+}_{0}(7)) + \text{dim}\mathcal{M}_{2\ell + 4}(\Gamma^{+}_{0}(7)) -1\\
        =& 2\left(\left\lfloor\left.\frac{\ell}{2}\right\rfloor\right. + \left\lfloor\left.\frac{\ell+1}{2}\right\rfloor\right. + \left\lfloor\left.\frac{\ell+2}{2}\right\rfloor\right.\right) + \left\lfloor\left.\frac{2\ell}{3}\right\rfloor\right. + \left\lfloor\left.\frac{2\ell+2}{3}\right\rfloor\right. + \left\lfloor\left.\frac{2\ell+4}{3}\right\rfloor\right. -3\ell -1.
    \end{split}
\end{align}

\subsubsection*{\texorpdfstring{$\ell=0$}{Lg}}
Consider the simple case with no poles $\ell = 0$ and two characters. The MLDE in this case reads
\begin{align}
    \left[\mathcal{D}^{2} + \phi_{1}(\tau)\mathcal{D} +  \phi_{0}(\tau) \right]f(\tau) = 0,
\end{align}
where $\phi_{0}(\tau)$ and $\phi_{1}(\tau)$ are modular forms of weights $4$ and $2$ respectively. Since there exists no weight $2$ modular form that belongs to the space of modular forms corresponding to the Fricke group $\Gamma_{0}^{+}(7)$, the MLDE simplifies to 
\begin{align}\label{MLDE_n=2}
    \left[\mathcal{D}^{2} + \phi_{0}(\tau)\right]f(\tau) = 0.
\end{align}
We now have three unique choices for $\phi_{0}(\tau)$, namely
\begin{align}\label{choices_phi}
    \begin{split}
        \phi_{0}(\tau) =& \mu E^{(7^{+})}_{4}(\tau) = \mu\Theta_{4,7}(\tau)\\
        =& \mu\left(1 + \tfrac{24}{5}q + \tfrac{216}{5}q^{2} + \tfrac{672}{5}q^{3} + \tfrac{1752}{5}q^{4} + \ldots\right)\\
        \phi_{0}(\tau) =& \mu \Theta^{2}_{2,7}(\tau) = \mu\theta_{7}^{4}(\tau)\\
        =& \mu\left(1 + 8q + 40q^{2} + 128q^{3} + 328q^{4} + \ldots\right)\\
        \phi_{0}(\tau) =& \mu\Delta_{7^{+},4}(\tau) = \mu\theta_{7}(\tau)j_{7}^{-1}(\tau)\mathbf{k}(\tau)\\
        =& \mu\left(q - q^{2} - 2q^{3} - 7q^{4} + \ldots\right).
    \end{split}
\end{align}
Here $\mu$ is a free parameter which will be fixed later. The space $\mathcal{M}_{4}\left(\Gamma_{0}^{+}(7)\right)$ is one-dimensional and we notice that all three of the above choices can be generated by $\Theta_{2,7}^{2}(\tau)$ and $\Theta_{4,7}(\tau)$ as shown below
\begin{align}
    \begin{split}
        E_{4}^{7^{+}}(\tau) =& a\Theta_{2,7}^{2} + b\Theta_{4,7}(\tau),\ a = 0,b = 1\\
        \Delta_{7^{+},4}(\tau) =& a\Theta_{2,7}^{2}(\tau) + b\Theta_{4,7}(\tau),\ a = \frac{5}{16},\ b = -\frac{5}{16}.
    \end{split}
\end{align}
Lastly, we note that $E_{4}^{(7^{+})}(\tau)$ is a quasi-modular form unlike $\Theta_{2,7}^{2}(\tau)$ (which is a modular form) since it transforms as follows under a modular transformation $\gamma = \tfrac{a\tau + b}{c\tau + d}$,
\begin{align}
    \begin{split}
        E_{k}(p\gamma(\tau)) =& (c\tau + d)^{2}E_{k}(p\tau) + \frac{12c}{2\pi ip}(c\tau + d),\\
        E_{4}^{(7^{+})}(\gamma(\tau)) =& (c\tau + d)^{2}E_{4}^{(7^{+})}(\tau) + \frac{48c}{25}\frac{(c\tau + d)}{2\pi i}.
    \end{split}
\end{align}
Hence, we only consider the second choice for $\phi_{0}(\tau)$ for our calculation. From the basis \ref{Fricke_basis}, we find
\begin{align}
    \begin{split}
        \mathcal{M}_{4}(\Gamma_{0}^{+}(7)) =& \theta_{7}(\tau)\left(\mathbb{C}\theta_{7}^{3}\oplus\mathbf{k}\mathbf{t}\right)\\
        =& \mathbb{C}\Theta_{2,7}^{2}\oplus\mathbb{C}\theta_{7}\mathbf{k}\mathbf{t}.
    \end{split}
\end{align}
Hence, the most general choice for $\phi_{0}(\tau)$ would be
\begin{align}
    \phi_{0}(\tau) =  \mu_{1}\Theta_{2,7}^{2}(\tau) + \mu_{2}\left(\theta_{7}\mathbf{k}\mathbf{t}\right)(\tau).
\end{align}
We now have two free parameters which matches with the result of \ref{number_of_parameters_F} for $\ell = 0$. Now, since the covariant derivative transforms a weight $r$ modular form into one of weight $r+2$, the double covariant derivative of a weight $0$ form is
\begin{align}
    \begin{split}
        \mathcal{D}^{2} = \mathcal{D}_{(2)}\mathcal{D}_{(0)} =& \left(\frac{1}{2\pi i}\frac{d}{d\tau} - \frac{1}{6}E_{2}(\tau)\right)\frac{1}{2\pi i}\frac{d}{d\tau}\\
        =& \Tilde{\partial}^{2} - \frac{1}{6}E_{2}(\tau)\Tilde{\partial}.
    \end{split}
\end{align}
The MLDE \ref{MLDE_n=2} now reads
\begin{align}
    \left[\Tilde{\partial}^{2} - \frac{1}{6}E_{2}(\tau)\Tilde{\partial} + \phi_{0}(\tau)\right]f(\tau) =0.
\end{align}
This equation can be solved by making the following mode expansion substitution for the character $f(\tau)$ and the Eisenstein series $E_{k}(\tau)$, and modular forms $\Theta_{2,7}^{2}(\tau)$ and $\left(\theta_{7}\mathbf{k}\mathbf{t}\right)(\tau)$,
\begin{align}\label{series_defs}
    \begin{split}
    f(\tau) =& q^{\alpha}\sum\limits_{n= 0}^{\infty}f_{n}q^{n},\\
    E_{k}(\tau) =& \sum\limits_{n=0}^{\infty}E_{k,n}q^{n},\\ \Theta_{2,7}^{2}(\tau) =& \sum\limits_{n=0}^{\infty}\Theta_{n}q^{n}\\
    =& 1 + 8 q + 40 q^2 + 128 q^3 + 328 q^4 + \ldots,\\
    \left(\theta_{7}\mathbf{k}\mathbf{t}\right)(\tau) =& \sum\limits_{n=0}^{\infty}\mathfrak{a}_{n}q^{n}\\
    =& 0 + q - q^2 - 2 q^3 - 7 q^4 + \ldots\\
    \end{split}
\end{align}
Substituting these expansions in the MLDE, we get
\begin{align}\label{MLDE_series_expressions}
    q^{\alpha}\sum\limits_{n=0}^{\infty}f_{n}q^{n}\left[\left(n + \alpha\right)^{2} + \sum\limits_{m=0}^{\infty}\left(\mu_{1}\Theta_{m} + \mu_{2}\mathfrak{a}_{m} - \frac{(n+\alpha)}{6}E_{2,m}\right)q^{m}\right] = 0.
\end{align}
We first restrict ourselves to the case when $\mu_{1} = \mu \neq 0$ and $\mu_{2} = 0$.
When $n=0, m=0$, with $E_{2,0} = 1 = \Theta_{0}$, we get the indicial equation
\begin{align}\label{alpha_eqn}
    \begin{split}
        &\alpha^{2} - \frac{\alpha}{6} + \mu = 0,\\
        &\alpha_{0} = \frac{1}{12}\left(1 -\sqrt{1 + 144\mu}\right) \equiv \frac{1}{12}\left(1 - x\right),\\
        &\alpha_{1} = \frac{1}{12}\left(1+\sqrt{1 + 144\mu}\right)\equiv \frac{1}{12}(1+x)
    \end{split}
\end{align}
where we set $x = +\sqrt{1 + 144\mu}$. The smaller solution $\alpha_{0} = \tfrac{1}{12}(1-x)$ corresponds to the identity character which behaves as $f(\tau) \sim q^{\tfrac{1-x}{12}}\left(1 + \mathcal{O}(q)\right)$. From \ref{character_behaviour}, the identity character $\chi_{0}$, associated with a primary of weight $\Delta_{0} = 0$ behaves as $\chi_{0}\sim q^{-\tfrac{c}{24}}\left(1 + \mathcal{O}(q)\right)$. Comparing the two behaviours, we obtain the following expression for the central charge
\begin{align}
    c = 2(x-1).
\end{align}
To find the conformal dimension $\Delta$, we compare the behaviours with the larger solution for $\alpha$, i.e. $f(\tau)\sim q^{\tfrac{1 + x}{12}}\left(1  +\mathcal{O}(q)\right)$ and $\chi\sim q^{-\tfrac{c}{24} + \Delta}\left(1 + \mathcal{O}(q)\right)$. This gives us
\begin{align}
    \Delta = \frac{x}{6}.
\end{align}
Next, to obtain a recurrence relation among the coefficients $f_{n}$, we use Cauchy product of two infinite series which reads
\begin{align}
    \left(\sum\limits_{i=0}^{\infty}\alpha_{i}\right)\cdot\left(\sum\limits_{j=0}^{\infty}\beta_{j}\right) = \sum\limits_{k=0}^{\infty}\gamma_{k},\ \gamma_{k} = \sum\limits_{p=0}^{k}\alpha_{p}\beta_{k-p}.
\end{align}
This gives us
\begin{align}\label{product_formulae}
    \begin{split}
        \left(\sum\limits_{m=0}^{\infty}E_{2,m}q^{m}\right)\left(\sum\limits_{n=0}^{\infty}f_{n}q^{n}(n+\alpha)\right) =& \sum\limits_{k=0}^{\infty}\left(\sum\limits_{p=0}^{k}E_{2,p}(k+\alpha - p)f_{k-p}\right)q^{k}\\
        \left(\sum\limits_{m=0}^{\infty}\Theta_{m}(\tau)q^{m}\right)\left(\sum\limits_{n=0}^{\infty}f_{n}q^{n}\right) =& \sum\limits_{k=0}^{\infty}\left(\sum\limits_{p=0}^{k}\Theta_{p}f_{k-p}\right)q^{k}.
    \end{split}
\end{align}
Relabelling and substituting this back into the MLDE, we get
\begin{align}
    \begin{split}
        q^{\alpha}\sum\limits_{n=0}^{\infty}q^{n}\left((n+\alpha)^{2} - \frac{(n+\alpha)}{6}E_{2,0} + \mu \Theta_{0}\right)f_{n} = q^{\alpha}\sum\limits_{n=0}^{\infty}q^{n}&\left(\sum\limits_{m=1}^{n}\left(\frac{1}{6}E_{2,m}(n+\alpha - m) - \mu\Theta_{m}\right)f_{n-m}\right).
    \end{split}
\end{align}
With $E_{k,0} = 1 = \Theta_{0}$ and \ref{alpha_eqn}, we get
\begin{align}\label{recursion_l=0}
    f_{n} = \left(n^{2} + 2\alpha n - \frac{n}{6}\right)^{-1}\sum\limits_{m=1}^{n}\left(\frac{1}{6}E_{2,m}(n+\alpha - m) - \mu\Theta_{m}\right)f_{n-m}.
\end{align}
When $n=1$ and $\alpha = \alpha_{0} = \tfrac{1}{12}(1-x)$, this simplifies to the following expression
\begin{align}
    \begin{split}
        m_{1}^{(0)}\equiv \frac{f_{1}^{(0)}}{f_{0}^{(0)}} = \frac{x^{2}+6x+7}{3(6-x)},
    \end{split}
\end{align}
where we used $E_{2,1} = -24$ and $\Theta_{1}= 8$. Solving for $x$, we obtain 
\begin{align}
    x = \frac{1}{2}\left(-(3m_{1} + 6) \pm \sqrt{(3m_{1}+6)^{2} + 4(18m_{1} + 7)}\right).
\end{align}
Since $2(x-1)$ is the central charge of the theory, $x$ must be rational. With $m_{1}^{(0)} = m_{1}$ and using the fact that $m_{1}$ is an integer, we conclude that at least one of the roots is rational. We now write
\begin{align}\label{to_be_recast}
    (3m_{1} + 18)^{2} - 260 = k^{2},
\end{align}
where $k\in\mathbb{Z}$. Defining
\begin{align}
    p \equiv 18 + 3m_{1} - k, 
\end{align}
we can recast \ref{to_be_recast} as follows
\begin{align}
   3m_{1} + 18 = \frac{p^{2} +260}{2p} = \frac{130}{p} + \frac{p}{2}.
\end{align}
This tells us that $p$ must be even, and that it must divide $130$. Restricting $k$ to be positive, we see that we have $k\geq 3m_{1}$ which implies that $p<18$. We conclude that all possible values of $m_{1}$ are found by those values of $p$ below $18$ that divide $130$ and that are even. The list of these values is $p = 2,10$. Table \ref{tab:theory_Fricke} contains CFT data among other things that correspond to particular theories.
\begin{table}[htb!]
    \centering
    \begin{tabular}{c|c|c|c|c}
    $p$ & $\mu$ & $m_{1}$ & $c$ & $\Delta$\\
    \hline & & & & \\
    2  & $\tfrac{1}{6}$ & 16 & 8 & $\tfrac{5}{6}$\\
    10 & $0$ & 0 & 0 & $\tfrac{1}{6}$\\
    \end{tabular}
    \caption{$c$ and $\Delta$ data corresponding to the Fricke group $\Gamma_{0}^{+}(7)$ for the choice $\phi_{0} = \mu\Theta_{2,7}^{2}(\tau)$ with $\ell = 0$.}
    \label{tab:theory_Fricke}
\end{table}
$m_{1}$ being non-negative is not sufficient proof to convince ourselves that this data might indeed be related to a CFT. Hence, we compute $m_{2}$ using recursion relation \ref{recursion_l=0}. If this turns out to be negative or fractional, then we rule out the theory as a viable candidate. We $n = 2$, we get
\begin{align}
    m_{2}^{(i)} \equiv \frac{f_{2}^{(i)}}{f_{0}^{(i)}} = -\frac{12(9\alpha_{i} + 10\mu)}{12\alpha_{i} + 11} - \frac{12m_{1}^{(i)}(3\alpha_{i} + 3 + 2\mu)}{12\alpha_{i} + 11}.
\end{align}
For $i = 0$, we find the values of $m_{2}^{(0)}$ corresponding to our candidate theories to yield $0$ for $p = 10$ and a negative fraction for $p = 2$ which we rule out. Now, we proceed to check if $m_{3}^{(i)}$ is positive as well for the surviving candidate theory. For $n = 3$, the recursion relation \ref{recursion_l=0} yields
\begin{align}
     m_{3}^{(i)} \equiv \frac{f_{3}^{(i)}}{f_{0}^{(i)}} = -\frac{32(3\alpha_{i} + 8\mu)}{12\alpha_{i} + 17} - \frac{8m_{1}^{(i)}(9\alpha_{i} + 9 + 10\mu)}{12\alpha_{i} + 17} - \frac{8m_{2}^{(i)}(3\alpha_{i} + 6 + 2\mu)}{12\alpha_{i} + 17}.
\end{align}
For $i = 0$, we obtain $m_{3}^{(0)} = \tfrac{224}{39}$ which is fractional and thus, we rule out this theory. We have found that there exists no CFT at $n = 2$ and $\ell = 0$.\\\\

\noindent For the case of $\mu_{1}\neq 0$ and $\mu_{2} \neq 0$, from \ref{MLDE_series_expressions} we find the following expressions for the free parameters by matching order by order in $q$
\begin{align}
    \begin{split}
        \mathcal{O}(1):&\ \mu = \frac{n + \alpha_{i}}{6} - (n + \alpha_{i}),\\
        \mathcal{O}(q):&\ \mu_{2} = \frac{8}{3}\left(3\alpha_{i}^{2} - 2\alpha_{i}\right).
    \end{split}
\end{align}
for $i=0,1$. When $i=0$, $\alpha_{0} = -\tfrac{c}{24}$ and this fixes
\begin{align}
    \mu_{1} = -\frac{c(c+4)}{576},\ \mu_{2} = \frac{c^{2}+16c}{72}.
\end{align}
From \ref{central_charge_valence_Fricke}, for $n = 2,\ \ell = 0$, we have $-\tfrac{c}{12} + \Delta = \tfrac{2}{3}$ which fixes the conformal dimension to be $\Delta = \tfrac{8 + c}{12}$. But it turns out that this case too yields inadmissible solutions. This makes sense since the parameter $\mu_{2}$ is one that is associated with a cusp form which, as we have seen in multiple instances in this work, is notorious for rendering the solutions to be inadmissible.

